Wilson lines and their Laurent positivity

For a marked surface $\Sigma$ and a semisimple algebraic group $G$ of adjoint type, we study the Wilson line morphism $g_{[c]}:\mathcal{P}_{G,\Sigma} \to G$ associated with the homotopy class of an arc $c$ connecting boundary intervals of $\Sigma$, which is the comparison element of pinnings via parallel-transport. The matrix coefficients of the Wilson lines give a generating set of the function algebra $\mathcal{O}(\mathcal{P}_{G,\Sigma})$ when $\Sigma$ has no punctures. The Wilson lines have the multiplicative nature with respect to the gluing morphisms introduced by Goncharov--Shen [GS19], hence can be decomposed into triangular pieces with respect to a given ideal triangulation of $\Sigma$. We show that the matrix coefficients $c_{f,v}^V(g_{[c]})$ give Laurent polynomials with positive integral coefficients in the Goncharov--Shen coordinate system associated with any decorated triangulation of $\Sigma$, for suitable $f$ and $v$.

==> LaurentTrace_sec6.tex <==
%---------------------New Section--------------------------------

\section{Network expansion formulae }\label{sec:network}
In this section, we give a diagrammatic way to compute the Wilson lines and Wilson loops in the natural representation of $\lie$ using the \emph{networks}. 

\subsection{Wilson lines and Wilson loops on positive real parts}
First let us clarify the functions which we will deal with. 
\begin{conv}
For a map $f: V_1 \to V_2$ between varieties with positive structures (\emph{e.g.} those coming from cluster structures), we denote the induced map on the positive real part by $f^+:V_1(\pos) \to V_2(\pos)$. 
\end{conv}

Let $\Sigma$ be a marked surface. 
A $G$-local system on $\Sigma$ is \emph{positive} if it admits a framing which makes it a point of the positive real part $\X_{G,\Sigma}(\pos)$. 
Recall that a free loop $|\gamma| \in \hat{\pi}(\Sigma)$ is said to be \emph{peripheral} if it is homotopic to a puncture, and otherwise \emph{essential}. 
Analogously, we say that a morphism $[c]: E_\inn \to E_\out$ in $\Pi_1^{\partial}(\Sigma)$ is \emph{peripheral} if it is homotopic to an interval in $\partial \Sigma$ which contains exactly one marked point, and otherwise \emph{essential}. Note that the free homotopy class of a essential automorphism $[\gamma] \in \pi_1(\Sigma,x)$ with $x \in E_\inn$ can be a peripheral loop. 
%Let $H_0 \subset H$ be the subvariety where the Weyl group $W(G)$ acts without fixed points (corresponding to the union of Weyl chambers). An element of $G(\mathbb{R})$ is called \emph{positive hyperbolic} if it is conjugated to an element of $H_0(\pos)$ (corresponding to the fundamental Weyl chamber). 
The following theorem is a variant of \cite[Theorem 1.9]{FG03}, which can be proved by a similar argument:

\begin{thm}
Let $G$ be a semisimple algebraic group of adjoint type. 
For any positive real point $(\L,\beta;p) \in \P_{G,\Sigma}(\pos)$, the Wilson lines give rise to a faithful functor $g_\bullet(\L,\beta;p): \Pi_1^{\partial}(\Sigma) \to G(\mathbb{R})$. Moreover the Wilson line $g_{[c]}(\L,\beta;p)$ along a morphism $[c]:E_\inn \to E_\out$ belongs to $G(\pos)$ if $[c]$ is essential, and otherwise does to $B^\pm(\pos)$.  
%Then the monodromy homomorphism of a positive $G$-local system induces an injective homomorphism $\rho_s: \pi_1(\Sigma,x_0) \to G(\mathbb{R})$. Moreover its monodromy along any essential loop is positive hyperbolic. 
\end{thm}
Thus we get a real-analytic function $g_{[c]}^+: \P_{G,\Sigma}(\pos) \to G(\pos)$ if $[c]$ is essential, and otherwise $g_{[c]}^+: \P_{G,\Sigma}(\pos) \to B^\pm(\pos)$.

Let $V$ be the natural representation of the Lie algebra $\lie=\mathrm{Lie}(G)$. Although it cannnot be integrated to a representation of the adjoint group $G$, $V^{\otimes k}$ can be integrated for some integer $k \geq 0$. For instance, for $G=PSL_{n+1}$ and the natural representation $V=\C^{n+1}$ of its Lie algebra $\mathfrak{sl}_{n+1}$, the tensor power $V^{\otimes n+1}$ is a well-defined $G$-module since any $(n+1)$-st root of unity acts trivially by Schur's lemma. 

Let us take a basis $\ket{1},\dots,\ket{\dim V}$ of $V$ which satisfies (P2), (P3) in \cref{t:positivechoice}, and let $\bra{1},\dots,\bra{\dim V}$ denote the dual basis.  
Then for a positive element $g \in G(\pos)$ or $B^\pm(\pos)$, its matrix coefficients on this representation is positive. Therefore we can consider the $k$-th root
\begin{align*}
    \bra{\alpha}g\ket{\beta}:= \sqrt[k]{c_{\bra{\alpha}^{\otimes k}, \ket{\beta}^{\otimes k}}^{V^{\otimes k}}(g^{\otimes k})}.
\end{align*}
What we are going to compute is such absolute values of the matrix coefficients
\begin{align*}
    \bra{\alpha}g_{[c]}^+)\ket{\beta} : \P_{G,\Sigma}(\pos) \to \pos
\end{align*}
of Wilson lines along morphisms $[c]: E_\inn \to E_\out$, and the trace
\begin{align*}
    \mathrm{tr}_V(\rho_{|\gamma|}^+):=\sum_{\alpha=1}^{\dim V}\bra{\alpha}\rho_{|\gamma|}^+\ket{\alpha}: \X_{G,\Sigma}(\pos) \to \pos
\end{align*}
of Wilson loops along free loops $|\gamma| \in \hat{\pi}(\Sigma)$. 

As in \cref{sec:monodromy,sec:coordinates}, let us first work on the side pairings. Let $\Pi$ be a polygon equipped with an ideal triangulation $\Delta$, $(E_\inn,E_\out)$ a pair of its sides, and $\tau_\Delta(E_\inn,E_\out)=(\tau_1,\dots,\tau_M) \in \{L,R\}^M$ the associated turning pattern. 
Recall the map $b_\nu: \P_{G,T_\nu} \to B^\pm$ from \cref{subsec:coordinate comparison}, which is defined as $b_\nu=b_{\tau_\nu}\circ f_{m_\nu}$. By \cref{t:coweight-GS} it is a positive map, and hence induces a map $b_\nu^+: \P_{G,T_\nu}(\pos) \to B^\pm(\pos)$. 
% For a reduced word $\bs$ of $w_0$ and $1\leq i \leq j \leq \dim V$, let us consider the function $\Delta_{\alpha\beta}^L: (\Conf_3 \P_G)(\pos) \to \pos$ given by the composition
% \begin{align}\label{eq:positive b_L}
%     \Delta_{\alpha\beta}^L: (\Conf_3 \P_G)(\pos) \xrightarrow{b_L^+} B^+(\pos) \xrightarrow{\Delta_{\alpha\beta}^V} \pos.
% \end{align}
% Similarly we consider the composition 
% \begin{align}\label{eq:positive b_R}
%     \Delta_{\alpha\beta}^R: (\Conf_3 \P_G)(\pos) \xrightarrow{b_R^+} B^-(\pos) \xrightarrow{\Delta_{\alpha\beta}^V} \pos.
% \end{align}
Then the following lemma is obtained from \cref{p:mon-decomp} by restricting each function to the positive real part:

\begin{lem}\label{l:positive_decomp}
Let the notations as above. Then we have
\begin{align*}
    \bra{\alpha}q_{\Delta}^*g_{E_\inn,E_\out}^+\ket{\beta} = \sum_{\alpha_1,\dots,\alpha_{M-1}=1}^{\dim V} \bra{\alpha}b_1^+\ket{\alpha_1}\bra{\alpha_1}b_2^+\ket{\alpha_2}\cdots \bra{\alpha_{M-1}}b_M^+\ket{\alpha}.
\end{align*}
\end{lem}
Now our aim is to give certain combinatorial expansion formulae for the functions $\bra{\alpha}(\psi_\bs^+)^*b_L^+\ket{\beta}$ $\bra{\alpha}(\psi_\bs^+)^*b_R^+\ket{\beta}$ via \emph{networks}, where $\psi_\bs^+: \mathbb{R}_{>0}^{I_\infty(\bs)} \xrightarrow{\sim} (\Conf_3 \P_G)(\pos)$ is induced by the GS coordinate system associated with a reduced word $\bs$ of $w_0$. 

(POSSIBLY MOVED TO INTRODUCTION)
Our general strategy is the following. Given a complex Lie algebra $\lie$ of classical type and a reduced word $\bs=(s_1,\dots,s_N)$ of the longest element $w_0 \in W(\lie)$, we will construct two oriented graphs $\cN_L(\lie,\bs)$ and $\cN_R(\lie,\bs)$ drawn on a plane (with a certain branching in the $D_n$ case), which we call the \emph{basic networks}. Its chambers are assigned the GS coordinates on $\Conf_3 \P_G$. 
The construction is carried out type-by-type in \cref{subsec:basic network}. 
To a certain edge path called a \emph{network path} in each basic network, we assign a monomial of GS coordinates on $\Conf_3 \P_G$ called the \emph{weight} so that these weights are precisely the monomials appearing in the Laurent polynomial $\psi_\bs^*f_{m_\nu}^*\Delta_{\alpha\beta}^{\tau_\nu}$. 
Then the Laurent polynomial $\psi_{\bD}^*\Delta_{\alpha\beta}^V(g_{E_\inn,E_\out}^+)$ can be expanded as a sum of weights for network paths in a network $\cN_{\bD}(E_\inn,E_\out)$ obtained by concatenating the basic networks according to the turning pattern. See \cref{subsec:closed network}. 

\subsection{Basic networks}\label{subsec:basic network}
In this subsection, we construct the basic networks $\cN_L(\lie,\bs)$ and $\cN_R(\lie,\bs)$ for a classical Lie algebra $\lie$ and a reduced word $\bs=(s_1,\dots,s_N)$ of the longest element $w_0 \in W(\lie)$. Although the construction depends on the type of $\lie$, they have the following common features:
\begin{itemize}
    \item Both $\cN_L(\lie,\bs)$ and $\cN_R(\lie,\bs)$ have horizontal lines $\ell_{\ket{\alpha}}$, each oriented from the right to the left, corresponding to the basic vector $\ket{\alpha}$ of the natural representation $V$. The right (resp. left) end point of $\ell_{\ket{\alpha}}$ is labeled as $\ell^+_{\ket{\alpha}}$ (resp. $\ell^-_{\ket{\alpha}}$).
    \item The network $\cN_L(\lie,\bs)$ (resp. $\cN_R(\lie,\bs)$) has vertical lines $\ell_1,\dots,\ell_N$ (resp. $\widetilde{\ell}_1,\dots,\widetilde{\ell}_N$) appearing in this order (resp. in the reversed order) from the left to the right, each oriented from the top to the bottom (resp. from the bottom to the top) and connecting two of horizontal lines. 
\end{itemize}
Depending on the type of $\lie$, these networks may have additional vertical lines. A \emph{network path} of type $(\alpha,\beta)$ in the basic network $\cN_*(\lie,\bs)$ with $* \in \{L,R\}$ is an edge path $\omega$ which starts from $\ell^+_{\ket{\beta}}$ and proceeds following the orientations of edges and arrives at $\ell^-_{\ket{\alpha}}$. The set of networks paths of type $(\alpha,\beta)$ in $\cN_\ast(\lie,\bs)$ is denoted by $P_{\alpha\beta}^\ast$ for $\ast \in \{L,R\}$. Let $\bX=(X_{s \choose i})_{(s,i) \in I_\infty(\bs)}$ denote the GS coordinates on $\Conf_3 \P_G$, and  $\mathbb{X}_s:=\prod_{i=0,\dots,n^s(\bs)} X_{s \choose i}$ for $s \in S$. 

\subsubsection{Type $A_n$ case}
Let $\lie=\mathfrak{sl}_{n+1}$. 
Take the natural representation $V=\C^{n+1}$ in which we have the following data:
\begin{description}
\item[Chevalley generators]
\begin{align*}
    e_s:=E_{s,s+1}, \quad f_s:=E_{s+1.s}, \quad \alpha_s^\vee:=E_{ss} - E_{s+1,s+1}.
\end{align*}
Here $E_{\alpha\beta}$ denote the $(n+1)\times (n+1)$-elementary matrix defined by $(E_{\alpha\beta})_{\alpha'\beta'}:=\delta_{\alpha\alpha'}\delta_{\beta\beta'}$. 
\item[Cartan matrix]
\begin{align*}
    C(A_n)=
    \begin{pmatrix} 
    2&-1& & & \\
    -1&2&-1& & \\
     &-1&\ddots& & & \\
     & & &2&-1\\
     & & &-1&2
    \end{pmatrix}.
\end{align*}
\item[One-parameter subgroups of $G=PSL_{n+1}$]
\begin{align}
    x_s(t) &= \exp(te_s) = \mathbbm{1}_{n+1} + tE_{s,s+1} \label{eq:x_s A_n}\\
    y_s(t) &= \exp(tf_s) = \mathbbm{1}_{n+1} + tE_{s+1,s} \label{eq:y_s A_n}\\
    H^s(x) &=\mathrm{diag}(\underbrace{x^{\frac{n+1-s}{n+1}},\dots,x^{\frac{n+1-s}{n+1}}}_{s},x^{-\frac{s}{n+1}},\dots,x^{-\frac{s}{n+1}}) =x^{-\frac{s}{n+1}} \cdot \overline{H^s}(x)
\end{align}
for $t,x >0$. Here $\mathbbm{1}_{n+1}$ denotes the identity matrix of size $n+1$, and the normalization $\overline{H^s}(x):=\mathrm{diag}(\underbrace{x,\dots,x}_{s},1,\dots,1)$ is useful in the sequel. 
\end{description}


% The column vectors of the inverse matrix $C(A_n)^{-1} = (\mathbf{c}_1,\dots,\mathbf{c}_n)$ is given by
% \begin{align*}
%     \mathbf{c}_s = \frac{1}{n+1}((n-s+1),2(n-s+1),\dots,\overset{(s-1)}{(s-1)(n-s+1)},\overset{(s)}{s(n-s+1)},s(n-s),\dots,s)^T.
% \end{align*}

Let $\ket{1},\dots,\ket{n+1}$ be the standard basis of $V$,  %$\epsilon_1,\dots,\epsilon_{n+1}$, 
where $\ket{1}$ is the highest weight vector and we have $\ket{\alpha+1}=f_\alpha\ket{\alpha}$ for $\alpha=1,\dots,n$. 

For a reduced word $\bs=(s_1,\dots,s_N)$ of $w_0$ (here $N=n(n+1)/2$), the basic network $\cN_L(A_n,\bs)$ is defined by letting the vertical line $\ell_k$ connect the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$ for $k=1,\dots,N$. 
% \begin{itemize}
%     \item It has $n+1$ horizontal lines  $\ell_{\ket{1}},\dots,\ell_{\ket{n+1}}$, each oriented from the right to the left. The right (resp. left) endpoint of $\ell_{\ket{j}}$ is denoted by $\ell_{\ket{j}}^+$ (resp. $\ell_{\ket{j}}^-$).  
%     \item It has vertical lines $\ell _1,\dots,\ell _N$, appearing in this order from the left to the right and oriented from the top to the bottom, where the line $\ell _k$ connects the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$. 
% \end{itemize}
An example for $n=4$ is shown in \cref{fig:network A_n}. 
We assign the GS coordinate $X_{s \choose i}$ on $\Conf_3 \P_G$ to the chamber sectioned by two horizontal lines $\ell_{\ket{s}}$ and $\ell_{\ket{s+1}}$, and the vertical lines $\ell _{k(s,i)}$ and $\ell _{k(s,i+1)}$. The chamber is unbounded if only one of these vertical lines exists. For a network path $\omega$, its \emph{weight} $wt_\omega: \R_{>0}^{I_\infty(\bs)} \to \pos$ is defined as the product of the GS coordinates assigned to the chambers above $\omega$. 

\begin{figure}
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
\fill[fillred] (9,4) -- (3,4) -- (3,3) -- (2,3) -- (2,2) -- (-1,2) -- (-1,5) -- (9,5) --cycle;
\foreach \i in {1,2,3,4,5}
\draw[->] (9,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-1,\i) node[left]{$\ell^-_{\ket{\i}}$};
%Vertical lines
\draw[<-] (1,1) node[below]{$\ell_1 $} -- (1,2);
\draw[<-] (2,2) -- (2,3);
\draw[<-] (3,3) -- (3,4);
\draw[<-] (4,4) -- (4,5);
\draw[<-] (3,1) -- (3,2);
\draw[<-] (4,2) -- (4,3);
\draw[<-] (5,3) -- (5,4);
\draw[<-] (5,1) -- (5,2);
\draw[<-] (6,2) -- (6,3);
\draw[<-] (7,1) node[below]{$\ell_{10} $} -- (7,2);
%Variables
\foreach \i in {0,1,2,3,4}
\draw (2*\i,1.5) node{$X_{1 \choose \i}$};
\foreach \i in {0,1,2,3}
\draw (2*\i+1,2.5) node{$X_{2\choose \i}$};
\foreach \i in {0,1,2}
\draw (2*\i+2,3.5) node{$X_{3 \choose \i}$};
\foreach \i in {0,1}
\draw (2*\i+3,4.5) node{$X_{4 \choose \i}$};
%A path
\draw[red,thick] (9,4) node[below left]{$\omega$} -- (3,4) -- (3,3) -- (2,3) -- (2,2) -- (-1,2);
\end{scope}
\end{tikzpicture}}
    \caption{The basic network $\cN_L(A_4,\bs)$ for $\bs=(1,2,3,4,1,2,3,1,2,1)$. A path $\omega \in P_{24}$ is shown in red.}
    \label{fig:network A_n}
\end{figure}

\begin{figure}
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
\fill[fillred] (9,2) -- (3,2) -- (3,3) -- (2,3) -- (2,4) -- (-1,4) -- (-1,5) -- (9,5)--cycle;
\foreach \i in {1,2,3,4,5}
\draw[->] (9,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-1,\i) node[left]{$\ell^-_{\ket{\i}}$};
%Vertical lines
\draw[->] (1,4) -- (1,5) node[above]{$\widetilde{\ell}_{10} $};
\draw[->] (2,3) -- (2,4);
\draw[->] (3,2) -- (3,3);
\draw[->] (4,1) -- (4,2);
\draw[->] (3,4) -- (3,5);
\draw[->] (4,3) -- (4,4);
\draw[->] (5,2) -- (5,3);
\draw[->] (5,4) -- (5,5);
\draw[->] (6,3) -- (6,4);
\draw[->] (7,4) -- (7,5) node[above]{$\widetilde{\ell}_1 $};
%Variables
\foreach \i in {0,1,2,3,4}
\draw (-2*\i+8,4.5) node{$X_{1 \choose \i}$};
\foreach \i in {0,1,2,3}
\draw (-2*\i+7,3.5) node{$X_{2\choose \i}$};
\foreach \i in {0,1,2}
\draw (-2*\i+6,2.5) node{$X_{3 \choose \i}$};
\foreach \i in {0,1}
\draw (-2*\i+5,1.5) node{$X_{4 \choose \i}$};
%A path
\draw[red,thick] (9,2) node[below left]{$\omega$} -- (3,2) -- (3,3) -- (2,3) -- (2,4) -- (-1,4);
\end{scope}
\end{tikzpicture}}
    \caption{The basic network $\cN_R(A_4,\bs)$ for $\bs^\ast_\op=(4,3,4,2,3,4,1,2,3,4)$. A path $\omega \in P_{24}$ is shown in red.}
    \label{fig:network A_n op}
\end{figure}

%For $1\leq i, j \leq n+1$, let $|\Delta_{\alpha\beta}|$ denote the coordinate function on $PGL_{n+1}(\pos) \cong PSL_{n+1}(\pos)$ taking the absolute value of the $(i,j)$-th component. 

\begin{lem}\label{l:network_left type_A}
We have
\begin{align*}
     \bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX)\ket{\beta} = \sfh_{A_n}(\mathbb{X}) \cdot \sum_{\omega \in P^L_{\alpha\beta}} wt_\omega(\bX) \quad \mbox{on $\R_{>0}^{I_\infty(\bs)}$},
\end{align*}
where $\sfh_{A_n}(\mathbb{X}):=\prod_{s=1}^n \mathbb{X}_s^{-\frac{s}{n+1}}$. 
\end{lem}

\begin{proof}
Recall the expression $b_L= u_+h_2$ from \cref{c:LR}. In the notation \eqref{eq:GS-standard}, it is written as $\psi_\bs^*b_L(\bX)=\sfu_+(\bX)\sfh_2(\bX)$.
We have
\begin{itemize}
    \item $\sfh_2(\bX) = \prod_{s=1}^n H^s(\mathbb{X}_s) = \sfh_{A_n}(\mathbb{X})\cdot \prod_{s=1}^n \overline{H^s}(\mathbb{X}_s)$ from \cref{l:Cartan-GS}, and
    \item $\sfu_+(\bX) = x_{s_1}(t_1)\dots x_{s_N}(t_N)$ with $t_{k(s,i)} = X_{s \choose 0}\dots X_{s \choose i-1}$ from \eqref{eq:Lus-GS}.
\end{itemize}
Let $\sfh'_2(\mathbb{X}):=\prod_{s=1}^n \overline{H^s}(\mathbb{X}_s)$. 
Then the matrix coefficient of $b_L$ is computed as
\begin{align*}
    \frac{1}{\sfh_{A_n}(\mathbb{X})} \bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX) \ket{\beta} = \bra{\alpha} x_{s_1}(t_1)\dots x_{s_N}(t_N)\sfh'_2(\mathbb{X})\ket{\beta} = \sum_{\omega \in P^L_{\alpha\beta}} wt_\omega^\Lus(\bX),
\end{align*}
where the weight $wt_\omega^\Lus(\bX)$ is defined to be the product of $\prod_{s \geq j} \mathbb{X}_s$ and the Lusztig parameters $t_k$ such that the path $\omega$ traverses the vertical line $\ell_k $. 

The diagrammatic explanation is the following. 
See \cref{fig:network A_n}. Imagine that the path $\omega$ emanates from the right endpoint $\ell^+_{\ket{\beta}}$ accompanied with the basis vector $\ket{\beta}$, and then moves along the network. First it encounters the matrix $\sfh'_2(\bX)$, and the accompanying vector is get multiplied with the scalar $\prod_{s \geq j} \mathbb{X}_s$. Observe from \eqref{eq:x_s A_n} that the action of $x_s(t_{k(s,i)})$ on basis vectors are given by
\begin{align*}
    x_s(t_{k(s,i)}): \quad
    \ket{s+1} &\mapsto \ket{s+1} + t_{k(s,i)} \ket{s}, \\
    \ket{\delta} &\mapsto \ket{\delta} \quad (\delta \neq s+1).
\end{align*}
Once the path $\omega$ accompanied with a vector proportional to $\ket{s+1}$ arrives at the top of a vertical line $\ell_{k(s,i)}$, either it goes left with its accompanying vector unchanged, or goes down with its accomanying vector changed to $t_{k(s,i)} \ket{s}$. If $\omega \in P^L_{\alpha\beta}$, then it is finally accompanied with a vector proportional to $\ket{\alpha}$. 
In this way the paths in $P^L_{\alpha\beta}$ exactly corresponds to the monomials in $x_{s_1}(t_1)\dots x_{s_N}(t_N)$. 

With a notice that $t_{k(s,i)} = X_{s \choose 0}\dots X_{s \choose i-1}$ is the product of all the variables assigned to the chambers on the left of the vertical line $\ell_s $, we see that $wt_\omega^\Lus(\bX) = wt_\omega(\bX)$ for all $\omega \in P^L_{\alpha\beta}$. Thus we get the desired formula. 
\end{proof}



\begin{ex}
Consider the path $\omega$ shown in red in \cref{fig:network A_n}. It traverses the vertical lines $\ell_2 =\ell_{k(2,1)} $ and $\ell_3 =\ell_{k(3,1)} $, and hence
\begin{align*}
    wt_\omega(\bX)=t_{k(2,1)}t_{k(3,1)}\mathbb{X}_4 =X_{2\choose 0}X_{3\choose 0}X_{4\choose 0}X_{4\choose 1}.
\end{align*}
\end{ex}

Next, let us consider the basic network $\cN_R(A_n,\bs)$. Let $\bs^\ast_{\op}=(s_N^\ast,\dots,s_1^\ast)$. The basic network $\cN_R(\A_n,\bs)$ is defined by letting the vertical line $\widetilde{\ell}_k$ connect the horizontal lines $\ell_{\ket{s_k^\ast}}$ and $\ell_{\ket{s_k^\ast+1}}$ for $k=1,\dots,N$.
% \begin{itemize}
%     \item It has the same horizontal lines  $\ell_{\ket{1}},\dots,\ell_{\ket{n+1}}$ as $\cN_L(A_n,\bs)$. 
%     \item It has vertical lines $\widetilde{\ell} _1,\dots,\widetilde{\ell} _N$, appearing in this order \emph{from the right to the left} and oriented from the bottom to the top, where the line $\widetilde{\ell} _k$ connects the horizontal lines $\ell_{\ket{s_k^\ast}}$ and $\ell_{\ket{s_k^\ast+1}}$. 
% \end{itemize}
An example for $n=4$ is shown in \cref{fig:network A_n op}. 
We assign the GS coordinate $X_{s \choose i}$ on $\Conf_3 \P_G$ to the chamber sectioned by two horizontal lines $\ell_{\ket{s^\ast}}$ and $\ell_{\ket{s^\ast+1}}$, and the vertical lines $\widetilde{\ell}_{k(s,i)}$ and $\widetilde{\ell} _{k(s,i+1)}$ (if exist). The chamber is unbounded if one of these lines is missing. For a network path $\omega$, its \emph{weight} $wt_\omega: \R_{>0}^{I_\infty(\bs)} \to \pos$ is defined as the product of the GS coordinates assigned to the chambers above $\omega$.

\begin{lem}\label{l:network_right type_A}
We have
\begin{align*}
    \bra{\alpha}(\psi_\bs^+)^*b_R^+\ket{\beta} = \sfh_{A_n}^\ast(\mathbb{X}) \cdot  \sum_{\omega \in P^R_{\alpha\beta}} wt_\omega(\bX) \quad \mbox{on $\R_{>0}^{I_\infty(\bs)}$},
\end{align*}
where $\sfh_{A_n}^\ast(\mathbb{X}):=\prod_{s=1}^n \mathbb{X}_{s^\ast}^{-\frac{s}{n+1}} = \prod_{s=1}^n \mathbb{X}_{s}^{-\frac{n+1-s}{n+1}}$.
\end{lem}

\begin{proof}
We follow the proof of \cref{l:network_left type_A} with the comparison relation $b_R = \vw^{-1} (u_+h_2)^{-1} \vw$ from \cref{c:LR}. Using \cref{l:generator_involution}, we get 
\begin{itemize}
    \item $\vw^{-1} \sfh_2(\bX)^{-1} \vw = \prod_{s=1}^n H^{s^\ast}(\mathbb{X}_s) = \prod_{s=1}^n H^{s}(\mathbb{X}_{s^\ast}) = \sfh_{A_n}^\ast(\mathbb{X}) \cdot \prod_{s=1}^n \overline{H^{s}}(\mathbb{X}_{s^\ast})$
    
    \item $\vw^{-1} \sfu_+(\bX)^{-1} \vw = y_{s_N^\ast}(t_N) \dots y_{s_1^\ast}(t_1)$ with $t_{k(s,i)} = X_{s \choose 0}\dots X_{s \choose i-1}$. Note that $\bs_\op^\ast=(s_N^\ast,\dots,s_1^\ast)$.
\end{itemize}
Letting $\widetilde{\sfh}'_2(\mathbb{X}):=\prod_{s=1}^n \overline{H^{s}}(\mathbb{X}_{s^\ast})$, the matrix coefficient of $b_R$ is computed as
\begin{align*}
    \frac{1}{\sfh_{A_n}^\ast(\mathbb{X})}\bra{\alpha}(\psi_\bs^+)^* b_R^+(\bX)\ket{\beta} = \bra{\alpha}\widetilde{\sfh}'_2(\mathbb{X}) y_{s_N^\ast}(t_N) \dots y_{s_1^\ast}(t_1)\ket{\beta} = \sum_{\omega \in P^R_{\alpha\beta}} \widetilde{wt}_\omega^\Lus(\bX),
\end{align*}
where the weight $\widetilde{wt}_\omega^\Lus(\bX)$ is defined to be the product of $\prod_{s \geq i} \mathbb{X}_{s^\ast}$ and the Lusztig parameters $t_k$ such that the path $\omega$ traverses the vertical line $\widetilde{\ell}_k $. 
This follows from the same diagrammatic reasoning as that in the proof of \cref{l:network_left type_A} with a notice that the action of $y_{s^\ast}(t_{k(s,i)})$ on basis vectors is given by
\begin{align*}
    y_{s^\ast}(t_{k(s,i)}): \ket{s^\ast} &\mapsto \ket{s^\ast} + t_{k(s,i)}\ket{s^\ast+1}, \\
    \ket{\delta} &\mapsto \ket{\delta} \quad (\delta\neq s^\ast)
\end{align*}
from \eqref{eq:y_s A_n}. 
Since $t_{k(s,i)}=X_{s \choose 0}\dots X_{s \choose i-1}$ is the product of all the variables assigned to the chambers on the right of the vertical line $\widetilde{\ell}_{k(s,i)} $, we see that $\widetilde{wt}_\omega^\Lus(\bX) = wt_\omega(\bX)$ for all $\omega \in P^R_{\alpha\beta}$. Thus we get the desired formula.
\end{proof}

\begin{ex}
Consider the path $\omega$ shown in red in \cref{fig:network A_n op}. It traverses the vertical lines $\widetilde{\ell}_7 =\widetilde{\ell}_{k(3,2)} $ and $\widetilde{\ell}_9 =\widetilde{\ell}_{k(2,3)} $, and hence
\begin{align*}
    \widetilde{wt}_\omega(\bX)=t_{k(3,2)}t_{k(2,3)}\mathbb{X}_{4^\ast} =X_{3\choose 0}X_{3\choose 1}X_{2\choose 0}X_{2\choose 1}X_{2\choose 2}X_{1\choose 0}X_{1\choose 1}X_{1\choose 2}X_{1\choose 3}X_{1\choose 4}.
\end{align*}
\end{ex}

\subsubsection{Type $C_n$ case}
Let $\lie=\mathfrak{sp}_{2n}$. Consider the symplectic form $J$ on the vector space $V=\C^{2n}$ given by $J=J_{2n}=\begin{pmatrix} 0 & I_n \\ -I_n & 0 \end{pmatrix}$ with the $n\times n$-matrix
\begin{align*}
    I_n:=\begin{pmatrix}
       &      &     &    1\\
       &      &   -1&     \\
       &\mbox{\reflectbox{$\ddots$}}&     & \\
 (-1)^n&      &     &     
    \end{pmatrix}.
\end{align*}
Then $\lie=\mathfrak{sp}_{2n}=\{X \in M_{2n}(\C) \mid X^TJ+JX = 0\}$ is represented on $V$ and we get the following data:
\begin{description}
\item[Chevalley generators]
\begin{align*}
    &e_s:=E_{s,s+1}+E_{2n-s,2n+1-s}, \quad f_s:=E_{s+1,s}+E_{2n+1-s,2n-s}, \\
    &\alpha_s^\vee:=E_{ss}-E_{s+1,s+1} - (E_{2n+1-s,2n+1-s}-E_{2n-s,2n-s})
\end{align*}
for $1\leq s \leq n-1$, and 
\begin{align*}
    e_n:=E_{n,n+1}, \quad f_n:=E_{n+1,n}, \quad \alpha_n^\vee:=E_{nn}-E_{n+1,n+1}.
\end{align*}
\item[Cartan matrix]
\begin{align*}
    C(C_n)=
    \begin{pmatrix} 
    2&-1& & & \\
    -1&2&-1& & \\
     &-1&\ddots& & & \\
     & & &2&-2\\
     & & &-1&2
    \end{pmatrix}.
\end{align*}
\item[One-parameter subgroups of $G=PSp_{2n}$]
\begin{align}
    x_s(t) &= \exp (te_s)=
    \mathbbm{1}_{2n} + tE_{s,s+1} + tE_{2n-s,2n+1-s}
    %\mathbbm{1}_{2n} + tE_{n,n+1} & s=n,
    \label{eq:x_s C_n}\\
    y_s(t) &= \exp (tf_s) = 
    \mathbbm{1}_{2n} + tE_{s+1,s} + tE_{2n+1-s,2n-s} 
    %\mathbbm{1}_{2n} + tE_{n+1,n} & s=n,
    \label{eq:y_s C_n}\\
    H^s(x)
    &=\mathrm{diag}(\underbrace{x,\dots,x}_s,1,\dots,1;1,\dots,1,\underbrace{x^{-1},\dots,x^{-1}}_s) =x^{-1} \cdot \overline{H^s}(x) \label{eq:H_s C_n}
    %\mathrm{diag}(x^{1/2},\dots,x^{1/2};x^{-1/2},\dots,x^{-1/2}) = x^{-1/2}\overline{H^n}(x) 
\end{align}
with $\overline{H}^s(x):=\mathrm{diag}(\underbrace{x^2,\dots,x^2}_s,x,\dots,x;x,\dots,x,\underbrace{1,\dots,1}_s)$
% \begin{align}
%     x_n(t) &= \exp (te_n) = \mathbbm{1}_{2n} + tE_{n,n+1} \label{eq:x_n C_n}\\
%     y_s(t) &= \exp (tf_n) = \begin{cases}
%     \mathbbm{1}_{2n} + tE_{s+1,s} + tE_{2n+1-s,2n-s} & 1\leq s \leq n-1, \\
%     \mathbbm{1}_{2n} + tE_{n+1,n} & s=n,
%     \end{cases} \label{eq:y_n C_n}\\
%     H^s(x)
%     &=\begin{cases}\mathrm{diag}(\underbrace{x,\dots,x}_s,1,\dots,1;1,\dots,1,\underbrace{x^{-1},\dots,x^{-1}}_s) =x^{-1} \cdot \overline{H^s}(x) & 1\leq s\leq n-1,\\
%     \mathrm{diag}(x^{1/2},\dots,x^{1/2};x^{-1/2},\dots,x^{-1/2}) = x^{-1/2}\overline{H^n}(x) & s=n
%     \end{cases}
% \end{align}
for $1\leq s \leq n-1$, and
\begin{align}
    x_n(t) &= \exp (te_n) = \mathbbm{1}_{2n} + tE_{n,n+1} \label{eq:x_n C_n}\\
    y_n(t) &= \exp (tf_n) = \mathbbm{1}_{2n} + tE_{n+1,n} \label{eq:y_n C_n}\\
    H^n(x) &=\mathrm{diag}(x^{1/2},\dots,x^{1/2};x^{-1/2},\dots,x^{-1/2}) = x^{-1/2}\cdot\overline{H^n}(x)\label{eq:H_n C_n}
\end{align}
with $\overline{H^n}(x):= \mathrm{diag}(x,\dots,x;1,\dots,1)$.
\end{description}

Let $\ket{1},\dots,\ket{2n}$ denote the standard basis of $V$, where $\ket{1}$ is the highest weight vector and we have $\ket{\alpha+1}=f_j\ket{\alpha}$ and $\ket{n+\alpha+1}=f_{n-\alpha}\ket{n+\alpha}$ for $\alpha=1,\dots,n$.

For a reduced word $\bs=(s_1,\dots,s_N)$ of $w_0$ (here $N=n^2$), the basic network $\cN_L(C_n,\bs)$ is defined as follows:
\begin{itemize}
    \item Let the vertical line $\ell _k$ connect the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$ for $k=1,\dots,N$.
    \item Put an additional vertical line $\ell'_k$ whenever $s_k \neq n$ in the same horizontal coordinate as $\ell_k $, and let it connect the horizontal lines $\ell_{\ket{2n+1-s_k}}$ and $\ell_{\ket{2n-s_k}}$.
\end{itemize}
% \begin{itemize}
%     \item It has $2n$ horizontal lines  $\ell_{\ket{1}},\dots,\ell_{\ket{2n}}$, each oriented from the right to the left. The right (resp. left) endpoint of $\ell_{\ket{j}}$ is denoted by $\ell_{\ket{j}}^+$ (resp. $\ell_{\ket{j}}^-$).  
%     \item It has vertical lines $\ell_1,\dots,\ell_N$, appearing in this order from the left to the right, where the line $\ell _k$ connects the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$. Moreover we have an additional vertical line $\ell'_k$ whenever $s_k \neq n$ which has the same horizontal coordinate as $\ell_k $, connecting the horizontal lines $\ell_{\ket{2n+1-s_k}}$ and $\ell_{\ket{2n-s_k}}$. These vertical lines are oriented from the top to the bottom.
% \end{itemize}
An example for $n=3$ is shown in \cref{fig:network C_n}. 
We assign the GS coordinates on $\Conf_3 \P_G$ as follows:
\begin{enumerate}
    \item For $1 \leq s \leq n-1$, we assign $X_{s \choose i}$ to the following two chambers: the chamber sectioned by the lines $\ell_{\ket{s}}$, $\ell_{\ket{s+1}}$, $\ell_{k(s,i)}$ and $\ell_{k(s,i+1)}$; the chamber sectioned by the lines $\ell_{\ket{2n+1-s}}$, $\ell_{\ket{2n-s}}$, $\ell'_{k(s,i)}$ and $\ell'_{k(s,i+1)}$. 
    \item We assign $X_{n \choose i}$ to the chamber sectioned by the lines $\ell_{\ket{n}}$, $\ell_{\ket{n+1}}$, $\ell_{k(n,i)}$ and $\ell_{k(n,i+1)}$.  
\end{enumerate}
For a network path $\omega$, its \emph{weight} $wt_\omega: \R_{>0}^{I_\infty(\bs)} \to \pos$ is defined as the product of the GS coordinates assigned to the chambers above $\omega$. 

\begin{figure}
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
\fill[fillred] (10,5) -- (4,5) -- (4,4) -- (2,4) -- (2,3) -- (-2,3) -- (-2,6) -- (10,6) --cycle;
\fill[fillgreen] (10,2) -- (3,2) -- (3,1) -- (-2,1) -- (-2,6) -- (10,6) --cycle;
\foreach \i in {1,2,3,4,5,6}
\draw[->] (10,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i) node[left]{$\ell^-_{\ket{\i}}$};
%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[->](\i,2) -- (\i,1);
    \draw[->](\i+1,3) -- (\i+1,2);
    \draw[->](\i+2,4) -- (\i+2,3);
    \draw[->](\i,6) -- (\i,5);
    \draw[->](\i+1,5) -- (\i+1,4);
    }
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (3*\i-1.5,1.5) node{$X_{1 \choose \i}$};
    \draw (3*\i-0.5,2.5) node{$X_{2 \choose \i}$};
    \draw (3*\i+0.5,3.5) node{$X_{3 \choose \i}$};
    \draw (3*\i-0.5,4.5) node{$X_{2 \choose \i}$};
    \draw (3*\i-1.5,5.5) node{$X_{1 \choose \i}$};
    }
%A path
\draw[red,thick] (10,5) node[below left]{$\omega$} -- (4,5) -- (4,4) -- (2,4) -- (2,3) -- (-2,3);
\draw[mygreen,thick] (10,2) node[below left]{$\omega'$} -- (3,2) -- (3,1) -- (-2,1);
\end{scope}
\end{tikzpicture}}
    \caption{The basic network $\cN_L(C_3,\bs)$ for $\bs=(1,2,3,1,2,3,1,2,3)$. A path $\omega \in P^L_{35}$ (resp. a path $c' \in P^L_{12}$) is shown in red (resp. green).}
    \label{fig:network C_n}
\end{figure}

\begin{figure}
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
\fill[fillgreen] (10,3) -- (3,3) -- (3,4) -- (1,4) -- (1,5) -- (-2,5) -- (-2,6) -- (10,6) --cycle;
\foreach \i in {1,2,3,4,5,6}
\draw[->] (10,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i) node[left]{$\ell^-_{\ket{\i}}$};
%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[<-](\i+2,2) -- (\i+2,1);
    \draw[<-](\i+1,3) -- (\i+1,2);
    \draw[<-](\i,4) -- (\i,3);
    \draw[<-](\i+2,6) -- (\i+2,5);
    \draw[<-](\i+1,5) -- (\i+1,4);
    }
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (-3*\i+9.5,1.5) node{$X_{1 \choose \i}$};
    \draw (-3*\i+8.5,2.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+7.5,3.5) node{$X_{3 \choose \i}$};
    \draw (-3*\i+8.5,4.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+9.5,5.5) node{$X_{1 \choose \i}$};
    }
% %A path
% \draw[red,thick] (10,5) node[above left]{$\omega$} -- (4,5) -- (4,4) -- (2,4) -- (2,3) -- (-2,3);
\draw[mygreen,thick] (10,3) node[below left]{$\omega$} -- (3,3) -- (3,4) -- (1,4) -- (1,5) -- (-2,5);
\end{scope}
\end{tikzpicture}}
    \caption{The basic network $\cN_R(C_3,\bs)$ for $\bs_\op^\ast=(3,2,1,3,2,1,3,2,1)$. A path $\omega \in P^R_{53}$ is shown in green.}
    \label{fig:network C_n op}
\end{figure}

\begin{lem}\label{l:network_left type_C}
We have
\begin{align*}
     \bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX)\ket{\beta} = \sfh_{C_n}(\mathbb{X}) \cdot \sum_{\omega \in P^L_{\alpha\beta}} wt_\omega(\bX) \quad \mbox{on $\R_{>0}^{I_\infty(\bs)}$},
\end{align*}
where $\sfh_{C_n}(\mathbb{X}):=(\prod_{s=1}^{n-1} \mathbb{X}_s^{-1})\mathbb{X}_n^{-1/2}$.
\end{lem}

\begin{proof}
The proof is similar to \cref{l:network_left type_A}. The normalizations in \eqref{eq:H_s C_n} and \eqref{eq:H_n C_n} are chosen so that $\sfh_2=\sfh_{C_n}\cdot \sfh'_2$ with $\sfh'_2(\mathbb{X}):=\prod_{s=1}^n \overline{H^s}(\mathbb{X}_s)$. 
Then one can verify that the normalized matrix coefficient $\sfh_{C_n}(\mathbb{X})^{-1}\bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX)\ket{\beta}$ is given by the sum of the weights of the network paths $\omega \in P^L_{\alpha\beta}$ just as in the type $A_n$ case, with a notice that 
\begin{align*}
    \sfh'_2(\mathbb{X}) \ket{\delta} = \begin{cases} (\prod_{s=1}^{\delta-1} \mathbb{X}_s)(\prod_{s=\delta}^{n-1} \mathbb{X}_s)^2 \mathbb{X}_n \cdot\ket{\delta} & \mbox{if $1 \leq \delta \leq n$}, \\ \vspace{1mm}
    (\prod_{s=\delta-n}^{n-1}\mathbb{X}_s) \cdot\ket{\delta} & \mbox{if $n+1 \leq \delta \leq 2n$}
    \end{cases}
\end{align*}
and the path gets multiplied by $t_{k(s,i)}$ for $1 \leq s \leq n-1$ whenever it traverses either the vertical line $\ell_{k(s,i)}$ or $\ell'_{k(s,i)}$ from \eqref{eq:x_s C_n}. 
\end{proof}

\begin{ex}
Consider the paths $\omega$ and $\omega'$ shown in \cref{fig:network C_n}. The path $\omega$ starts from $\ell_{\ket{4}}^+$ and traverses the vertical lines $\ell_3=\ell_{k(3,1)}$ and $\ell'_5=\ell'_{k(2,2)}$, and hence
\begin{align*}
    wt_\omega(\bX) = t_{k(3,1)}t_{k(2,2)}\mathbb{X}_1 = X_{3 \choose 0}X_{2 \choose 0}X_{2 \choose 1}X_{1 \choose 0}X_{1 \choose 1}X_{1 \choose 2}X_{1 \choose 3}.
\end{align*}
The path $\omega'$ starts from $\ell_{\ket{2}}^+$ and traverses the vertical line $\ell_4=\ell_{k(1,1)}$, and hence
\begin{align*}
    wt_{\omega'}(\bX) = t_{k(1,1)}\mathbb{X}_1\mathbb{X}_2^2\mathbb{X}_3
\end{align*}
which is the product of all the GS coordinates except for $X_{1 \choose 2}$ and $X_{1 \choose 3}$.
\end{ex}
The basic network $\cN_R(C_n,\bs)$ is similarly defined. The relation between $\cN_L(C_n,\bs)$ and $\cN_R(C_n,\bs)$ is analogous to that in type $A_n$. Here note that the Dynkin involution is trivial in this case. An example of $\cN_R(C_n,\bs)$ corresponding to \cref{fig:network C_n} is shown in \cref{fig:network C_n op}. The network weight $wt_\omega$ for a network path $\omega$ in $\cN_R(C_n,\bs)$ is the product of the GS coordinates assigned to the chambers above $\omega$. Then similarly to \cref{l:network_right type_A}, we get
\begin{align*}
    \bra{\alpha}(\psi_\bs^+)^*b_R^+\ket{\beta} = \sfh_{C_n}(\mathbb{X}) \cdot  \sum_{\omega \in P^R_{\alpha\beta}} wt_\omega(\bX).
\end{align*}

\subsubsection{Type $B_n$ case}
Let $\lie=\mathfrak{so}_{2n+1}$. Consider the symmetric form 
\begin{align*}
    K=K_{2n+1}:=\left(\begin{array}{c|c|c}
      & &I_n\\ \hline
      &1&   \\ \hline
   I_n^T& &
    \end{array} \right)
\end{align*}
on $V=\C^{2n+1}$. 
Then $\lie=\mathfrak{so}_{2n+1}=\{X \in M_{2n+1}(\C)\mid X^TK + KX = 0\}$ is represented on $V$ and we get the following data:
\begin{description}
\item[Chevalley generators]
\begin{align*}
    &e_s:=E_{s,s+1} + E_{2n+1-s,2n+2-s}, \quad f_s:=E_{s+1,s} + E_{2n+2-s,2n+1-s}, \\
    &\alpha_s^\vee:=E_{ss}-E_{s+1,s+1} - (E_{2n+2-s,2n+2-s}-E_{2n+1-s,2n+1-s})
\end{align*}
for $1 \leq s \leq n-1$, and
\begin{align*}
    &e_n:=E_{n,n+1} + 2E_{n+1,n+2}, \quad
    f_n:=2E_{n+1,n} + E_{n+2,n+1}, \\
    &\alpha_n^\vee:=2(E_{nn}-E_{n+2,n+2}).
\end{align*}
\item[Cartan matrix]
\begin{align*}
    C(B_n)=
    \begin{pmatrix} 
    2&-1& & & \\
    -1&2&-1& & \\
     &-1&\ddots& & & \\
     & & &2&-1\\
     & & &-2&2
    \end{pmatrix}.
\end{align*}
\item[One-parameter subgroups of $G=SO_{2n+1}$]

\begin{align}
    x_s(t) &= \exp (te_s) = \mathbbm{1}_{2n+1} + t(E_{s,s+1} + E_{2n+1-s,2n+2-s}) \label{eq:x_s B_n}\\
    y_s(t) &= \exp (tf_s) = \mathbbm{1}_{2n+1} + t(E_{s+1,s} + E_{2n+2-s,2n+1-s}) \label{eq:y_s B_n} 
\end{align}
for $1\leq s \leq n-1$,
\begin{align}
    x_n(t) &= \exp (te_n) = \mathbbm{1}_{2n+1} + tE_{n,n+1} + 2tE_{n+1,n+2} + t^2E_{n,n+2} \label{eq:x_n B_n} \\
    y_n(t) &= \exp (tf_n) = \mathbbm{1}_{2n+1} + tE_{n+1,n} + 2tE_{n+2,n+1} + t^2E_{n+2,n}. \label{eq:y_n B_n}, 
\end{align}
and 
\begin{align}
    H^s(x)
    &=\mathrm{diag}(\underbrace{x,\dots,x}_s,1,\dots,1;1;1,\dots,1,\underbrace{x^{-1},\dots,x^{-1}}_s) =x^{-1} \cdot \overline{H^s}(x) \label{eq:H_s B_n}
\end{align}
with $\overline{H}^s(x):=\mathrm{diag}(\underbrace{x^2,\dots,x^2}_s,x,\dots,x;x;x,\dots,x,\underbrace{1,\dots,1}_s)$ for $1\leq s \leq n$.
\end{description}
Let $\ket{1},\dots,\ket{2n+1}$ denote the standard basis of $V$, where $\ket{1}$ is the highest weight vector and we have $\ket{\alpha+1}=f_\alpha\ket{\alpha}$ for $\alpha=1,\dots,n-1$, $\ket{n+1}=(1/2)f_n\ket{n}$ and $\ket{n+\alpha+1}=f_{n+1-\alpha}\ket{n+\alpha}$ for $\alpha=1,\dots,n$.

For a reduced word $\bs=(s_1,\dots,s_N)$ of $w_0$ (here $N=n^2$), the basic network $\cN_L(B_n,\bs)$ is defined as follows:
\begin{itemize}
    \item Let the vertical line $\ell_k$ connect the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$ for $k=1,\dots,N$.
    \item Put an additional vertical line $\ell'_k$ whenever $s_k \neq n$ at a position slightly right to $\ell_k$, and let it connect the horizontal lines $\ell_{\ket{2n+2-s_k}}$ and $\ell_{\ket{2n+1-s_k}}$. \item Put an additional vertical line $\ell''_k$ at a position slightly left to $\ell_k$, and let it connect the horizontal lines $\ell_{\ket{n+1}}$ and $\ell_{\ket{n-1}}$.
\end{itemize}
% \begin{itemize}
%     \item It has $2n+1$ horizontal lines $\ell_{\ket{1}},\dots,\ell_{\ket{2n+1}}$, each oriented from the right to the left. The right (resp. left) endpoint of $\ell_{\ket{j}}$ is denoted by $\ell_{\ket{j}}^+$ (resp. $\ell_{\ket{j}}^-$). 
%     \item It has vertical lines $\ell_1,\dots,\ell_N$, appearing in this order from the left to the right, where the line $\ell_k$ connects the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$. Moreover we have an additional vertical line $\ell'_k$ whenever $s_k \neq n$ which is located at a position slightly right to $\ell_k$ in the horizontal direction, connecting the horizontal lines $\ell_{\ket{2n+2-s_k}}$ and $\ell_{\ket{2n+1-s_k}}$. 
%     Whenever $s_k=n$, we have one more vertical line $\ell''_k$ which is located at a position slightly left to $\ell_k$ in the horizontal direction, connecting the horizontal lines $\ell_{\ket{n+1}}$ and $\ell_{\ket{n-1}}$. All these vertical lines are oriented from the top to the bottom. 
% \end{itemize}
The resulting network is regarded as an oriented \emph{planar} graph with the convention that at an intersection point of the type $\scalebox{0.7}{\begin{tikzpicture} 
    \begin{scope}[>=latex]
    \draw[->] (0.5,0) -- (-0.5,0);
    \draw[->,line width=5pt,draw=white] (0,0.5) -- (0,-0.5);
    \draw[->] (0,0.5) -- (0,-0.5);
    \end{scope}
    \end{tikzpicture}}$,
a network path is only allowed to go either from the north to the south or from the east to the west. A \emph{chamber} of $\cN_L(B_n,\bs)$ is a connected component of its complement as a planar graph. 
An example for $n=3$ is shown in \cref{fig:network B_n}.
We assign the GS coordinates on $\Conf_3 \P_G$ as follows:
\begin{enumerate}
    \item For $1 \leq s \leq n-1$, we assign $X_{s \choose i}$ to the following two chambers: the chamber sectioned by the lines $\ell_{\ket{s}}$, $\ell_{\ket{s+1}}$, $\ell_{k(s,i)}$ and $\ell_{k(s,i+1)}$; the chamber sectioned by $\ell_{\ket{2n+2-s}}$, $\ell_{\ket{2n+1-s}}$, $\ell'_{k(s,i)}$ and $\ell'_{k(s,i+1)}$.
    \item We assign $X_{n \choose i}$ (resp. $2X_{n \choose i}$) to the chamber sectioned by the lines $\ell_{\ket{n}}$, $\ell_{\ket{n+1}}$, $\ell''_{k(n,i)}$ and $\ell_{k(n,i+1)}$ (resp. sectioned by $\ell_{\ket{n+1}}$, $\ell_{\ket{n+2}}$, $\ell''_{k(n,i)}$ and $\ell'_{k(n,i+1)}$). 
    \item We assign an auxiliary scalar $1/2$ to the chamber sectioned by the lines $\ell_{\ket{n+1}}$, $\ell_{\ket{n+2}}$, $\ell'_{k(n,i)}$ and $\ell''_{k(n,i)}$ for $i=1,\dots,n^n(\bs)$. The remaining chambers are understood to be assigned the scalar $1$. 
\end{enumerate}
For a network path $\omega$, its \emph{weight} $wt_\omega: \R_{>0}^{I_\infty(\bs)} \to \pos$ is defined as the product of the GS coordinates assigned to the chambers above $\omega$. 
\begin{figure}
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
\fill[fillgreen] (10,5) -- (2.333,5) -- (2.333,3) -- (-2,3) -- (-2,7) -- (10,7) --cycle;
\foreach \i in {1,2,3,4,5,6,7}
\draw[->] (10,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i) node[left]{$\ell^-_{\ket{\i}}$};
%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[->](\i,2) -- (\i,1);
    \draw[->](\i+1,3) -- (\i+1,2);
    \draw[->](\i+2,4) -- (\i+2,3);
    \draw[->](\i+1.666,5) -- (\i+1.666,4);
    \draw[line width=5pt, shorten >=1pt, shorten <=1pt, draw=white](\i+2.333,5) -- (\i+2.333,3);
    \draw[->](\i+2.333,5) -- (\i+2.333,3);
    \draw[->](\i,7) -- (\i,6);
    \draw[->](\i+1,6) -- (\i+1,5);
    }
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (3*\i-1.5,1.5) node{$X_{1 \choose \i}$};
    \draw (3*\i-0.5,2.5) node{$X_{2 \choose \i}$};
    \draw (3*\i+0.5,3.5) node{$X_{3 \choose \i}$};
    \draw (3*\i+0.5,4.5) node{$2X_{3 \choose \i}$};
    \draw (3*\i-0.5,5.5) node{$X_{2 \choose \i}$};
    \draw (3*\i-1.5,6.5) node{$X_{1 \choose \i}$};
    }
\foreach \i in {0,1,2}
    \draw (3*\i+2,4.5) node{$\frac{1}{2}$};
%A path
\draw[red,thick] (10,6) node[below left]{$\omega$} -- (4,6) -- (4,5) -- (1.666,5) -- (1.666,4) -- (-2,4);
\draw[mygreen,thick] (10,5) node[above left]{$\omega'$} -- (2.333,5) -- (2.333,3) -- (-2,3);
\end{scope}
\end{tikzpicture}}
    \caption{The basic network $\cN_L(B_3,\bs)$ for $\bs=(1,2,3,1,2,3,1,2,3)$. A path $\omega \in P^L_{46}$ (resp. a path $\omega' \in P^L_{35}$) is shown in red (resp. green).}
    \label{fig:network B_n}
\end{figure}

\begin{figure}
\begin{tikzpicture}
\begin{scope}[>=latex]
\fill[fillgreen] (10,2) -- (7,2) -- (7,3) -- (6.333,3) -- (6.333,4) -- (-2,4) -- (-2,7) -- (10,7) --cycle;
\foreach \i in {1,2,3,4,5,6,7}
\draw[->] (10,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i) node[left]{$\ell^-_{\ket{\i}}$};
%Green path, latter half
\draw[mygreen,thick] (6.333,4) -- (-2,4);
%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[<-](\i+2,2) -- (\i+2,1);
    \draw[<-](\i+1,3) -- (\i+1,2);
    \draw[<-](\i+0.333,4) -- (\i+0.333,3);
    \draw[<-](\i+0.5,5) -- (\i+0.5,4);
    \draw[line width=5pt, shorten >=1pt, shorten <=1pt, draw=white](\i-0.333,5) -- (\i-0.333,3);
    \draw[<-](\i-0.333,5) -- (\i-0.333,3);
    \draw[<-](\i+2,7) -- (\i+2,6);
    \draw[<-](\i+1,6) -- (\i+1,5);
    }
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (-3*\i+9.5,1.5) node{$X_{1 \choose \i}$};
    \draw (-3*\i+8.5,2.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+7.5,3.5) node{$2X_{3 \choose \i}$};
    \draw (-3*\i+7.5,4.5) node{$X_{3 \choose \i}$};
    \draw (-3*\i+8.5,5.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+9.5,6.5) node{$X_{1 \choose \i}$};
    }
\foreach \i in {0,1,2}
    \draw (3*\i,3.5) node{$\frac{1}{2}$};
%Red path & Green path, former half
\draw[mygreen,thick] (10,2) node[above left]{$\omega'$} -- (7,2) -- (7,3) -- (6.333,3) -- (6.333,4);
\draw[red,thick] (10,3) node[above left]{$\omega$} -- (5.666,3) -- (5.666,5) -- (-2,5);
\end{scope}
\end{tikzpicture}
    \caption{The basic network $\cN_R(B_3,\bs)$ for $\bs_\op^\ast=(3,2,1,3,2,1,3,2,1)$. A path $\omega \in P^R_{53}$ (resp. a path $\omega' \in P^R_{42}$) is shown in red (resp. green).}
    \label{fig:network B_n op}
\end{figure}


\begin{lem}\label{l:network_left type_B}
We have
\begin{align*}
     \bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX)\ket{\beta} = \sfh_{B_n}(\mathbb{X}) \cdot \sum_{\omega \in P^L_{\alpha\beta}} wt_\omega(\bX) \quad \mbox{on $\R_{>0}^{I_\infty(\bs)}$},
\end{align*}
where $\sfh_{B_n}(\mathbb{X}):=\prod_{s=1}^{n} \mathbb{X}_s^{-1}$.
\end{lem}

\begin{proof}
The proof is similar to \cref{l:network_left type_A}. The normalization in \eqref{eq:H_s B_n} is chosen so that $\sfh_2=\sfh_{B_n}\cdot \sfh'_2$ with $\sfh'_2(\mathbb{X}):=\prod_{s=1}^n \overline{H^s}(\mathbb{X}_s)$. 
Then one can verify that the normalized matrix coefficient $\sfh_{B_n}^{-1}\bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX)\ket{\beta}$ is given by the sum of the weights of the network paths $\omega \in P^L_{\alpha\beta}$ just as in the type $A_n$ case with a notice that 
\begin{align*}
    h'_2 \ket{\delta} = \begin{cases} (\prod_{s=1}^{\delta-1} \mathbb{X}_s)(\prod_{s=\delta}^{n-1} \mathbb{X}_s)^2 \mathbb{X}_n \cdot\ket{\delta} & \mbox{if $1 \leq \delta \leq n$}, \\ \vspace{1mm}
    (\prod_{s=1}^{n}\mathbb{X}_s)\cdot \ket{\delta} & \mbox{if $\delta=n+1$}, \\ \vspace{1mm}
    (\prod_{s=\delta-n-1}^{n-1}\mathbb{X}_s) \cdot\ket{\delta} & \mbox{if $n+2 \leq \delta \leq 2n+1$}
    \end{cases}
\end{align*}
and the path gets multiplied by $t_{k(s,i)}$ for $1 \leq s \leq n-1$ whenever it traverses either the vertical line $\ell_{k(s,i)}$ or $\ell'_{k(s,i)}$ from \eqref{eq:x_s B_n}. Moreover a special attention should be payed to the fact that the path $\omega$ gets multiplied by $t_{k(n,i)}$ (resp. $2t_{k(n,i)}$, $t_{k(n,i)}^2$)  whenever it traverses the vertical line $\ell_{k(n,i)}$ (resp. $\ell'_{k(n,i)}$, $\ell''_{k(n,i)}$) from \eqref{eq:x_n B_n}. 
\end{proof}

\begin{ex}
Consider the paths $\omega$ and $\omega'$ shown in \cref{fig:network B_n}. 
The path $\omega$ starts from $\ell_{\ket{6}}^+$ and traverses the vertical lines $\ell'_5=\ell'_{k(2,2)}$ and $\ell'_3 = \ell'_{k(3,1)}$, and hence
\begin{align*}
    wt_{c}(\bX) = 2t_{k(3,1)}t_{(k(2,2)}\mathbb{X}_1 = 2X_{3 \choose 0}X_{2 \choose 0}X_{2 \choose 1}X_{1 \choose 0}X_{1 \choose 1}X_{1 \choose 2}X_{1 \choose 3}.
\end{align*}
The path $\omega'$ starts from $\ell_{\ket{5}}^+$ and traverses the vertical line $\ell''_3=\ell''_{k(3,1)}$, and hence
\begin{align*}
    wt_{\omega'}(\bX) = t_{k(3,1)}\mathbb{X}_1\mathbb{X}_2 = X_{3 \choose 0}^2X_{2 \choose 0}X_{2 \choose 1}X_{2 \choose 2}X_{2 \choose 3}X_{1 \choose 0}X_{1 \choose 1}X_{1 \choose 2}X_{1 \choose 3}.
\end{align*}
Here the contribution $X_{3 \choose 0}^2$ can be understood as the product of the chamber variables $2X_{3 \choose 0}$, $X_{3 \choose 0}$, $1/2$ (and $1$). 
\end{ex}
The basic network $\cN_R(B_n,\bs)$ is similarly defined. The relations between $\cN_L(B_n,\bs)$ and $\cN_R(B_n,\bs)$ is analogous to that in type $A_n$, except that the Dynkin involution is trivial here. An example of $\cN_R(B_n,\bs)$ corresponding to \cref{fig:network B_n} is shown in \cref{fig:network B_n op}. The network weight $wt_\omega$ for a network path $\omega$ in $\cN_R(B_n,\bs)$ is the product of the GS coordinates assigned to the chambers above $\omega$. Then similarly to \cref{l:network_right type_A}, we get 
\begin{align*}
    \bra{\alpha}(\psi_\bs^+)^*b_R^+\ket{\beta} = \sfh_{B_n}(\mathbb{X}) \cdot  \sum_{\omega \in P^R_{\alpha\beta}} wt_\omega(\bX).
\end{align*}



\subsubsection{Type $D_n$ case}
Let $\lie=\mathfrak{so}_{2n}$. Consider the symmetric form 
\begin{align*}
    K=K_{2n}:=\begin{pmatrix} 0& I_n \\ I_n^T&0  \end{pmatrix}
    % =\begin{pmatrix}
    %   &      &      &     &    1\\
    %   &      &      &   -1&     \\
    %   &      &\mbox{\reflectbox{$\ddots$}}& & \\
    %   &-1    &      &      & \\
    %  1&      &      &      &     
    % \end{pmatrix}
\end{align*}
on $V=\C^{2n}$. 
Then $\lie=\mathfrak{so}_{2n}=\{X \in M_{2n}(\C)\mid X^TK + KX = 0\}$ is represented on $V$ and we get the following data:
\begin{description}
\item[Chevalley generators]
\begin{align*}
    e_s&:=E_{s,s+1} + E_{2n-s,2n+1-s}, \quad f_s:=E_{s+1,s} + E_{2n+1-s,2n-s}, \\
    \alpha_s^\vee&:=E_{ss}-E_{s+1,s+1} - (E_{2n+1-s,2n+1-s}-E_{2n-s,2n-s})
\end{align*}
for $1 \leq s \leq n-1$ and
\begin{align*}
    e_n&:=E_{n-1,n+1} + E_{n,n+2}, \quad f_n:=E_{n+1,n-1} + E_{n+2,n}, \\
    \alpha_n^\vee&:=E_{n-1,n-1} + E_{nn} - (E_{n+1,n+1} + E_{n+2,n+2}).
\end{align*}
\item[Cartan matrix]
\begin{align*}
    C(D_n)=
    \begin{pmatrix} 
    2&-1& & & & \\
    -1&2&-1& & & \\
     &-1&\ddots&\ddots& & & \\
     & &\ddots&2&-1&-1\\
     & & &-1&2& \\
     & & &-1& &2
    \end{pmatrix}.
\end{align*}
\item[One-parameter subgroups of $G=PSO_{2n}$]
\begin{align}
    x_s(t) &= \exp (te_s) = \mathbbm{1}_{2n} + t(E_{s,s+1} + E_{2n-s,2n+1-s}) \label{eq:x_s D_n}\\
    y_s(t) &= \exp (tf_s) = \mathbbm{1}_{2n} + t(E_{s+1,s} + E_{2n+1-s,2n-s}) \label{eq:y_s D_n}
\end{align}
for $1 \leq s \leq n-1$,
\begin{align}
    x_n(t) &= \exp (te_n) = \mathbbm{1}_{2n} + t(E_{n-1,n+1} + E_{n,n+2})\label{eq:x_n D_n}\\
    y_n(t) &= \exp (tf_n) = \mathbbm{1}_{2n} + t(E_{n+1,n-1} + E_{n+2,n}),\label{eq:y_n D_n}
\end{align}
\begin{align}
    H^s(x)
    =\mathrm{diag}(\underbrace{x,\dots,x}_s,1,\dots,1;1,\dots,1,\underbrace{x^{-1},\dots,x^{-1}}_s) =x^{-1} \cdot \overline{H^s}(x) \label{eq:H_s D_n}
\end{align}
with $\overline{H}^s(x):=\mathrm{diag}(\underbrace{x^2,\dots,x^2}_s,x,\dots,x;x,\dots,x,\underbrace{1,\dots,1}_s)$
for $1\leq s \leq n-1$,
\begin{align}
    H^{n-1}(x)
    =\mathrm{diag}(x^{1/2},\dots,x^{1/2},x^{-1/2};x^{1/2},x^{-1/2},\dots,x^{-1/2}) =x^{-1/2} \cdot \overline{H^{n-1}}(x)\label{eq:H_n-1 D_n}
\end{align}
with $\overline{H}^{n-1}(x):=\mathrm{diag}(x,\dots,x,1;x,1,\dots,1)$, and 
\begin{align}
    H^{n}(x)
    =\mathrm{diag}(x^{1/2},\dots,x^{1/2},x^{1/2};x^{-1/2},x^{-1/2},\dots,x^{-1/2}) =x^{-1/2} \cdot \overline{H^{n}}(x) \label{eq:H_n D_n}
\end{align}
with $\overline{H}^{n}(x):=\mathrm{diag}(x,\dots,x;1,\dots,1)$.
\end{description}
Let $\ket{1},\dots,\ket{2n}$ denote the standard basis of $V$, where $\ket{1}$ is the highest weight vector and we have $\ket{\alpha+1}=f_\alpha\ket{\alpha}$ for $\alpha=1,\dots,n-1$, $\ket{n+1}=f_n\ket{n-1}$, $\ket{n+\alpha+1}=f_{n-\alpha}\ket{n+\alpha}$ for $\alpha=1,\dots,n-1$. 

For a reduced word $\bs=(s_1,\dots,s_N)$ of $w_0$ (here $N=n(n-1)$), basic network $\cN_L(D_n,\bs)$ is defined as follows:
\begin{itemize}
    \item Let the vertical line $\ell_k$ connect the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$ if $s_k \neq n$; otherwise $\ell_{\ket{n+2}}$ and $\ell_{\ket{n}}$.
    \item Put an additional vertical line $\ell'_k$ for each $k=1,\dots,N$ in the same horizontal position as $\ell_k$. If $s_k \leq n-2$, it connects the horizontal lines $\ell_{\ket{2n+1-s_k}}$ and $\ell_{\ket{2n-s_k}}$; if $s_k=n-1$, it connects $\ell_{\ket{n+2}}$ and $\ell_{\ket{n+1}}$; if $s_k=n$, it connects $\ell_{\ket{n+1}}$ and $\ell_{\ket{n-1}}$.
\end{itemize}
% \begin{itemize}
%     \item It has $2n$ horizontal lines $\ell_{\ket{1}},\dots,\ell_{\ket{2n}}$, each oriented from the right to the left. The right (resp. left) endpoint of $\ell_{ket{j}}$ is denoted by $\ell_{\ket{j}}^+$ (resp. $\ell_{\ket{j}}^-$).
%     \item It has vertical lines $\ell_1,\dots,\ell_N$, appearing in this order from the left to the right, where the line $\ell_k$ connects the horizontal lines $\ell_{\ket{s_k+1}}$ and $\ell_{\ket{s_k}}$ when $s_k \neq n$; it connects $\ell_{\ket{n+2}}$ and $\ell_{\ket{n}}$ when $s_k=n$. Moreover we have an additional vertical line $\ell'_k$ for each $k=1,\dots,N$, which has the same horizontal coordinate as $\ell_k$. For $s_k \leq n-2$, it connects the horizontal lines $\ell_{\ket{2n+1-s_k}}$ and $\ell_{\ket{2n-s_k}}$; for $s_k=n-1$, it connects $\ell_{\ket{n+2}}$ and $\ell_{\ket{n+1}}$; for $s_k=n$, it connects $\ell_{\ket{n+1}}$ and $\ell_{\ket{n-1}}$. These vertical lines are oriented from the top to the bottom.
% \end{itemize}
An example for $n=4$ is shown in \cref{fig:network D_n}. Note that the network $\cN_L(D_n,\bs)$ can be naturally placed on a \lq\lq branched" surface $\Sigma_L$ obtained by patching two planes  $\Sigma_L^f=\Sigma_L^b = \mathbb{R}^2$ off a thin strip $\mathbb{R} \times (-1,1)$. The lines $\ell_{\ket{\alpha}}$ with $\alpha \neq n+1$ lie on the \lq\lq front" sheet $\Sigma_L^f$, and those with $\alpha \neq n$ on the \lq\lq back" sheet $\Sigma_L^b$. The corresponding branches of the network $\cN_L(D_n,\bs)$ are shown in \cref{fig:network D_n front-back}. 
We assign the GS coordinates on $\Conf_3 \P_G$ as follows:
\begin{enumerate}
    \item For $1 \leq s \leq n-2$, we assign $X_{s \choose i}$ to the following two chambers: the chamber sectioned by the lines $\ell_{\ket{s}}$, $\ell_{\ket{s+1}}$, $\ell_{k(s,i)}$ and $\ell_{k(s,i+1)}$; the one sectioned by $\ell_{\ket{2n+1-s}}$, $\ell_{\ket{2n-s}}$,$\ell'_{k(s,i)}$ and $\ell'_{k(s,i+1)}$.
    \item We assign $X_{n-1 \choose i}$ (resp. $X_{n \choose i}$) to the chamber in the front sheet $\Sigma_L^f$ sectioned by the lines $\ell_{\ket{n-1}}$, $\ell_{\ket{n}}$, $\ell_{k(n-1,i)}$ and $\ell_{k(n-1,i+1)}$ (resp. sectioned by $\ell_{\ket{n}}$, $\ell_{\ket{n+2}}$, $\ell_{k(n,i)}$ and $\ell_{k(n,i+1)}$).
    \item We also assign $X_{n-1 \choose i}$ (resp. $X_{n \choose i}$) to the chamber in the back sheet $\Sigma_L^b$ sectioned by the lines $\ell_{\ket{n+1}}$, $\ell_{\ket{n+2}}$, $\ell'_{k(n-1,i)}$ and $\ell'_{k(n-1,i+1)}$ (resp. sectioned by $\ell_{\ket{n-1}}$, $\ell_{\ket{n+1}}$, $\ell'_{k(n,i)}$ and $\ell'_{k(n,i+1)}$).
\end{enumerate}
Note that each network path $\omega$ traverses only one of the two sheets $\Sigma_L^f$ and $\Sigma_L^b$. Its \emph{weight} $wt_\omega: \R_{>0}^{I_\infty(\bs)} \to \pos$ is defined as the product of the GS coordinates assigned to the chambers above $\omega$ in that sheet. 

\begin{figure}
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
\fill[fillred] (11,5.5) -- (5,5.5) -- (4,4) -- (0.666,4) -- (1.666,3) -- (-2,3) -- (-3,4) -- (-2,5.5) -- (-2,7.5) -- (11,7.5) --cycle;
\foreach \i in {1,2,3}
\draw[->] (11,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i) node[left]{$\ell^-_{\ket{\i}}$};

\foreach \i in {6,7,8}
\draw[->] (11,\i-0.5) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i-0.5) node[left]{$\ell^-_{\ket{\i}}$};

\draw[->] (12,4.5) node[right]{$\ell^+_{\ket{5}}$} -- (-1,4.5) node[left]{$\ell^-_{\ket{5}}$};
%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[->](\i,2) -- (\i,1);
    \draw[->](\i+1,3) -- (\i+1,2);
    \draw[->](\i,8-0.5) -- (\i,7-0.5);
    \draw[->](\i+1,7-0.5) -- (\i+1,6-0.5);
    \draw[->](\i+3,4.5) -- (\i+2,3);
    \draw[->](\i+1.666,5.5) -- (\i+2.666,4.5);
    }
\draw[line width=5pt, shorten >=1pt, shorten <=1pt, draw=white] (10,4) -- (-3,4);
\draw[line width=5pt, shorten >=1pt, shorten <=1pt, fillred] (0.666,4) -- (-3,4);
\draw[->] (10,4) -- (-3,4);
    %\sarrow{10,4}{-3,4}
\draw(10,4) node[right]{$\ell^+_{\ket{4}}$};
\draw(-3,4) node[left]{$\ell^-_{\ket{4}}$};

\foreach \i in {0,3,6}
    {
    \sarrow{\i+2,5.5}{\i+1,4}
    \draw[->](\i+0.666,4) -- (\i+1.666,3);
    }
\draw[line width=5pt, shorten >=1pt, shorten <=1pt, draw=white] (2,5.5) -- (1,4);
    \draw[line width=5pt, shorten >=1pt, shorten <=1pt, fillred] (2,5.5) -- (1,4);
    \draw[->] (2,5.5) -- (1,4);
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (3*\i-1.5,1.5) node{$X_{1 \choose \i}$};
    \draw (3*\i-0.5,2.5) node{$X_{2 \choose \i}$};
    \draw (3*\i-0.5,6) node{$X_{2 \choose \i}$};
    \draw (3*\i-1.5,7) node{$X_{1 \choose \i}$};
    }
%A path
\draw[red,thick] (11,5.5) node[above left]{$\omega$} -- (5,5.5) -- (4,4) -- (0.666,4) -- (1.666,3) -- (-2,3);
%Names of lines
\draw (1,3.5) node[left]{$\ell_3$};
\draw (1,5) node[right]{$\ell_4$};
\draw (3,3.5) node[left]{$\ell'_4$};
\draw (3,5) node[left]{$\ell'_3$};
% \draw[mygreen,thick] (10,2) node[above left]{$\omega'$} -- (3,2) -- (3,1) -- (-2,1);
\end{scope}
\end{tikzpicture}}
    \caption{The basic network $\cN_L(D_4,\bs)$ for $\bs=(1,2,3,4)^3$. A path $\omega \in P^L_{36}$ is shown in red.}
    \label{fig:network D_n}
\end{figure}

\begin{figure}
\[
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
%-------------Top--------------------
\fill[fillred] (11,5) -- (5,5) -- (4,4) -- (0.666,4) -- (1.666,3) -- (-2,3) -- (-3,4) -- (-2,5) -- (-2,7) -- (11,7) --cycle;
\foreach \i in {1,2,3}
\draw[->] (11,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i) node[left]{$\ell^-_{\ket{\i}}$};

\foreach \i in {6,7,8}
\draw[->] (11,\i-1) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i-1) node[left]{$\ell^-_{\ket{\i}}$};

%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[->](\i,2) -- (\i,1);
    \draw[->](\i+1,3) -- (\i+1,2);
    \draw[->](\i,8-1) -- (\i,7-1);
    \draw[->](\i+1,7-1) -- (\i+1,6-1);
    %\draw[->](\i+3,4) -- (\i+2,3);
    %\draw[->](\i+1.666,5) -- (\i+2.666,4);
    }
\draw[line width=5pt, shorten >=1pt, shorten <=1pt, draw=white] (10,4) -- (-3,4);
\draw[line width=5pt, shorten >=1pt, shorten <=1pt, draw=fillred] (0.666,4) -- (-3,4);
\draw[->] (10,4) -- (-3,4);
    %\sarrow{10,4}{-3,4}
    \draw(10,4) node[right]{$\ell^+_{\ket{4}}$};
    \draw(-3,4) node[left]{$\ell^-_{\ket{4}}$};
\foreach \i in {0,3,6}
    {
    \sarrow{\i+2,5}{\i+1,4}
    \draw[->](\i+0.666,4) -- (\i+1.666,3);
    }
\draw[line width=5pt, shorten >=1pt, shorten <=1pt, draw=white] (2,5) -- (1,4);
    \draw[line width=5pt, shorten >=1pt, shorten <=1pt, fillred] (2,5) -- (1,4);
    \draw[->] (2,5) -- (1,4);
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (3*\i-1.5,1.5) node{$X_{1 \choose \i}$};
    \draw (3*\i-0.5,2.5) node{$X_{2 \choose \i}$};
    \draw (3*\i-0.5,3.5) node{$X_{3 \choose \i}$};
    \draw (3*\i-0.5,4.5) node{$X_{4 \choose \i}$};
    \draw (3*\i-0.5,5.5) node{$X_{2 \choose \i}$};
    \draw (3*\i-1.5,6.5) node{$X_{1 \choose \i}$};
    }
%A path
\draw[red,thick] (11,5) node[below left]{$\omega$} -- (5,5) -- (4,4) -- (0.666,4) -- (1.666,3) -- (-2,3);
%----------Bottom---------------------
{\begin{scope}[yshift=-8cm]
\fill[fillred] (11,5) -- (-2,5) -- (-2,7) -- (11,7) --cycle;
\foreach \i in {1,2,3}
\draw[->] (11,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i) node[left]{$\ell^-_{\ket{\i}}$};

\foreach \i in {6,7,8}
\draw[->] (11,\i-1) node[right]{$\ell^+_{\ket{\i}}$} -- (-2,\i-1) node[left]{$\ell^-_{\ket{\i}}$};

\draw[->] (12,4) node[right]{$\ell^+_{\ket{5}}$} -- (-1,4) node[left]{$\ell^-_{\ket{5}}$};
%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[->](\i,2) -- (\i,1);
    \draw[->](\i+1,3) -- (\i+1,2);
    \draw[->](\i,8-1) -- (\i,7-1);
    \draw[->](\i+1,7-1) -- (\i+1,6-1);
    \draw[->](\i+3,4) -- (\i+2,3);
    \draw[->](\i+1.666,5) -- (\i+2.666,4);
    }
% \sarrow{9,4}{-3,4}
%     \draw(9,4) node[right]{$\ell^+_{\ket{4}}$};
%     \draw(-3,4) node[left]{$\ell^-_{\ket{4}}$};
% \foreach \i in {0,3,6}
%     {
%     \sarrow{\i+2,5}{\i+1,4}
%     \draw[->](\i+0.666,4) -- (\i+1.666,3);
%     }
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (3*\i-1.5,1.5) node{$X_{1 \choose \i}$};
    \draw (3*\i-0.5,2.5) node{$X_{2 \choose \i}$};
    \draw (3*\i+1,3.5) node{$X_{4 \choose \i}$};
    \draw (3*\i+1,4.5) node{$X_{3 \choose \i}$};
    \draw (3*\i-0.5,5.5) node{$X_{2 \choose \i}$};
    \draw (3*\i-1.5,6.5) node{$X_{1 \choose \i}$};
    }
%A path
\draw[red,thick] (11,5) node[below left]{$\omega$} -- (5,5);
\end{scope}}
\end{scope}
\end{tikzpicture}}
\]
    \caption{The front (top) and back (bottom) branches of the network $\cN_L(D_4,\bs)$ for $\bs=(1,2,3,4)^3$.}
    \label{fig:network D_n front-back}
\end{figure}

\begin{figure}
\scalebox{0.9}{
\begin{tikzpicture}
\begin{scope}[>=latex]
%-------------Top--------------------
\fill[fillred] (10,2) -- (4,2) -- (4,3) -- (10,3) --cycle;
\fill[fillred] (10,5) -- (1,5) -- (1,6) -- (-3,6) -- (-3,7) -- (10,7) --cycle;
\foreach \i in {1,2,3}
\draw[->] (10,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-3,\i) node[left]{$\ell^-_{\ket{\i}}$};

\foreach \i in {6,7,8}
\draw[->] (10,\i-1) node[right]{$\ell^+_{\ket{\i}}$} -- (-3,\i-1) node[left]{$\ell^-_{\ket{\i}}$};

%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[<-](\i+2,2) -- (\i+2,1);
    \draw[<-](\i+1,3) -- (\i+1,2);
    \draw[<-](\i+2,8-1) -- (\i+2,7-1);
    \draw[<-](\i+1,7-1) -- (\i+1,6-1);
    %\draw[->](\i+3,4) -- (\i+2,3);
    %\draw[->](\i+1.666,5) -- (\i+2.666,4);
    }
\sarrow{9,4}{-4,4}
    \draw(9,4) node[right]{$\ell^+_{\ket{4}}$};
    \draw(-4,4) node[left]{$\ell^-_{\ket{4}}$};
\foreach \i in {0,3,6}
    {
    \sarrow{\i-1,4}{\i,5}
    \draw[<-](\i+0.666-2,4) -- (\i+1.666-2,3);
    }
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (-3*\i+9.5,1.5) node{$X_{1 \choose \i}$};
    \draw (-3*\i+8.5,2.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+7,3.5) node{$X_{4 \choose \i}$};
    \draw (-3*\i+7,4.5) node{$X_{3 \choose \i}$};
    \draw (-3*\i+8.5,5.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+9.5,6.5) node{$X_{1 \choose \i}$};
    }
%A path
\draw[red,thick] (10,2) node[above left]{$\omega$} -- (4,2) -- (4,3);
\draw[red,thick] (2.666,5) -- (1,5) -- (1,6) -- (-3,6);
%----------Bottom---------------------
{\begin{scope}[yshift=-8cm]
\fill[fillred] (10,2) -- (4,2) -- (4,3) -- (3,3) --(4,4) -- (3.666,4) -- (2.666,5) -- (1,5) -- (1,6) -- (-3,6) -- (-3,7) -- (10,7) -- (10,5) -- (11,4) -- (10,3) --cycle;
\foreach \i in {1,2,3}
\draw[->] (10,\i) node[right]{$\ell^+_{\ket{\i}}$} -- (-3,\i) node[left]{$\ell^-_{\ket{\i}}$};

\foreach \i in {6,7,8}
\draw[->] (10,\i-1) node[right]{$\ell^+_{\ket{\i}}$} -- (-3,\i-1) node[left]{$\ell^-_{\ket{\i}}$};

\draw[->] (11,4) node[right]{$\ell^+_{\ket{5}}$} -- (-2,4) node[left]{$\ell^-_{\ket{5}}$};
%Vertical lines
\foreach \i in {0,3,6}
    {
    \draw[<-](\i+2,2) -- (\i+2,1);
    \draw[<-](\i+1,3) -- (\i+1,2);
    \draw[<-](\i+2,8-1) -- (\i+2,7-1);
    \draw[<-](\i+1,7-1) -- (\i+1,6-1);
    \draw[<-](\i+1,4) -- (\i,3);
    \draw[<-](\i+1.666-2,5) -- (\i+0.666,4);
    }
% \sarrow{9,4}{-3,4}
%     \draw(9,4) node[right]{$\ell^+_{\ket{4}}$};
%     \draw(-3,4) node[left]{$\ell^-_{\ket{4}}$};
% \foreach \i in {0,3,6}
%     {
%     \sarrow{\i+2,5}{\i+1,4}
%     \draw[->](\i+0.666,4) -- (\i+1.666,3);
%     }
%Variables
\foreach \i in {0,1,2,3}
    {
    \draw (-3*\i+9.5,1.5) node{$X_{1 \choose \i}$};
    \draw (-3*\i+8.5,2.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+7.5,3.5) node{$X_{4 \choose \i}$};
    \draw (-3*\i+7.5,4.5) node{$X_{3 \choose \i}$};
    \draw (-3*\i+8.5,5.5) node{$X_{2 \choose \i}$};
    \draw (-3*\i+9.5,6.5) node{$X_{1 \choose \i}$};
    }
%A path
\draw[red,thick] (10,2) node[above left]{$\omega$} -- (4,2) -- (4,3) -- (3,3) --(4,4) -- (3.666,4) -- (2.666,5) -- (1,5) -- (1,6) -- (-3,6);
\end{scope}}
\end{scope}
\end{tikzpicture}}
    \caption{The basic network $\cN_R(D_4,\bs)$ for $\bs_\op^\ast=(3,4,2,1)^3$. The front (resp. back) sheet is shown in the top (resp. bottom). A path $\omega \in P^R_{72}$ is shown in red.}
    \label{fig:network D_n op}
\end{figure}


\begin{lem}\label{l:network_left type_D}
We have
\begin{align*}
     \bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX)\ket{\beta} = \sfh_{D_n}(\mathbb{X}) \cdot \sum_{\omega \in P^L_{\alpha\beta}} wt_\omega(\bX) \quad \mbox{on $\R_{>0}^{I_\infty(\bs)}$},
\end{align*}
where $\sfh_{D_n}(\mathbb{X}):=\left(\prod_{s=1}^{n-2} \mathbb{X}_s^{-1}\right) \mathbb{X}_{n-1}^{-1/2}\mathbb{X}_{n}^{-1/2}$.
\end{lem}

\begin{proof}
The proof is similar to \cref{l:network_left type_A}. The normalizations in \eqref{eq:H_s D_n}, \eqref{eq:H_n-1 D_n} and \eqref{eq:H_n D_n} are chosen so that $\sfh_2=\sfh_{D_n}\cdot \sfh'_2$ with $\sfh'_2(\mathbb{X}):=\prod_{s=1}^n \overline{H^s}(\mathbb{X}_s)$. 
Then one can verify that the normalized matrix coefficient $\sfh_{D_n}(\mathbb{X})^{-1}\bra{\alpha}(\psi_\bs^+)^*b_L^+(\bX)\ket{\beta}$ is given by the sum of the weights of the network paths $\omega \in P^L_{\alpha\beta}$ just as in the type $A_n$ case with a notice that 
\begin{align*}
    \sfh'_2(\mathbb{X}) \ket{\delta} = \begin{cases} (\prod_{s=1}^{\delta-1} \mathbb{X}_s)(\prod_{s=\delta}^{n-2} \mathbb{X}_s)^2 \mathbb{X}_{n-1}\mathbb{X}_n \cdot\ket{\delta} & \mbox{if $1 \leq\delta \leq n-2$}, \\ \vspace{1mm}
    \mathbb{X}_{n-1}\mathbb{X}_n\cdot \ket{\delta} & \mbox{if $\delta=n-1$}, \\ \vspace{1mm}
    \mathbb{X}_n \cdot\ket{\delta} & \mbox{if $\delta=n$}, \\ 
    (\prod_{s=1}^{n-2} \mathbb{X}_s)\mathbb{X}_{n-1} \cdot\ket{\delta} & \mbox{if $\delta=n+1$}, \\
    \vspace{1mm}
    (\prod_{s=1}^{2n-\delta} \mathbb{X}_s)\cdot \ket{\delta} & \mbox{if $n+2 \leq\delta \leq 2n$}.
    \end{cases}
\end{align*}
and the path gets multiplied by $t_{k(s,i)}$ for $1 \leq s \leq n$ whenever it traverses either the vertical line $\ell_{k(s,i)}$ or $\ell'_{k(s,i)}$ from \eqref{eq:x_s D_n} and \eqref{eq:x_n D_n}. 
\end{proof}

\begin{ex}
Consider the path $\omega$ shown in \cref{fig:network D_n}. The path $\omega$ starts from $\ell_{\ket{6}}^+$ and traverses the vertical lines $\ell_8=\ell_{k(4,2)}$ and $\ell_3=\ell_{k(3,1)}$, and hence
\begin{align*}
    wt_\omega(\bX) = t_{k(3,1)}t_{k(4,2)}\mathbb{X}_2\mathbb{X}_1 = X_{4 \choose 0}X_{4 \choose 1}X_{3 \choose 0}X_{2 \choose 0}X_{2 \choose 1}X_{2 \choose 2}X_{2 \choose 3}X_{1 \choose 0}X_{1 \choose 1}X_{1 \choose 2}X_{1 \choose 3}.
\end{align*}
\end{ex}
The basic network $\cN_R(D_n,\bs)$ is similarly defined. Note that the Dynkin involution exchanges the index $n-1$ and $n$. An example of $\cN_R(D_n,\bs)$ corresponding to \cref{fig:network D_n} is shown in \cref{fig:network D_n op}. The network weight $wt_\omega$ for a network path $\omega$ in $\cN_R(D_n,\bs)$ is defined similarly. Then similarly to \cref{l:network_right type_A}, we get
\begin{align*}
    \bra{\alpha}(\psi_\bs^+)^*b_R^+\ket{\beta} = \sfh_{D_n}(\mathbb{X}) \cdot  \sum_{\omega \in P^R_{\alpha\beta}} wt_\omega(\bX). 
\end{align*}
Finally, we give an interpretation of the exponents appearing in $\sfh_{\lie}(\mathbb{X})$. Let $C(\lie)^{-1}=(C^{st})_{s,t \in S}$ be the inverse of the Cartan matrix. 

\begin{lem}
For $\lie=A_n,B_n,C_n$ or $D_n$, we have $\sfh_\lie(\mathbb{X})=\prod_{s\in S}\mathbb{X}_s^{-C^{s,1^\ast}}$.
\end{lem}

\begin{proof}
Notice that in each case, our normalization $\sfh_2=\sfh_\lie\cdot \sfh'_2$ is made so that $\sfh'_2(\mathbb{X})$ acts on the lowest weight vector $v_{w_0\varpi_1}$ trivially. For any weight $\lambda$, we have
\begin{align*}
    \sfh_2(\mathbb{X}).v_{w_0\lambda}=\sfh_2(\mathbb{X})^{w_0\lambda}v_{w_0\lambda}=\left(\prod_{s\in S}H^s(\mathbb{X}_s)^{w_0\lambda}\right)v_{w_0\lambda}
    =\prod_{s \in S}\mathbb{X}_s^{\langle \varpi_s^\vee,w_0\lambda\rangle}v_{w_0\lambda}.
\end{align*}
Substituting $\lambda=\varpi_1$, we get $\sfh_\lie(\mathbb{X})=\prod_{s \in S}\mathbb{X}_s^{\langle \varpi_s^\vee,-\varpi_{1^\ast}\rangle} = \prod_{s \in S}\mathbb{X}_s^{-C^{s,1^\ast}}$.
\end{proof}

\subsection{Network expansion formulae}
Now we are going to give a network expansion formula for the matrix coefficients of the side pairing. 

Let $\Pi$ be a polygon equipped with an ideal triangulation $\Delta$, $(E_\inn,E_\out)$ a pair of its side edges, and $\tau_\Delta(E_\inn,E_\out) = (\tau_\nu)_{\nu=1}^M$ the associated turning pattern. Let $\bD:=(\Delta_*(E_\inn,E_\out),(\bs_\nu)_{\nu=1}^M)$. 
We concatenate the basic networks $\cN_{\tau_1}(\lie,\bs_1),\dots,\cN_{\tau_{M}}(\lie,\bs_{M})$ in this order from the left to the right, by matching the horizontal lines with the same basis labels. 
%We also glue the left-most endpoints of $\cN_{\tau_1}(\lie,\bs_1)$ to the right-most endpoints of $\cN_{\tau_M}(\lie,\bs_M)$ by matching the basis labels. 
%The resulting \lq\lq closed" oriented graph $\cN_{\bD}(E_\inn,E_\out)$ is called the \emph{network associated with the pair $(E_\inn,E_\out)$ and the reduced words $\bs_1,\dots,\bs_M$}. 
In this process, certain pairs of chambers are merged. To a new chamber arising in this way, we assign the product of GS coordinates which have been assigned to the chambers merged together. Then from the definition of the GS coordinates by amalgamation, the chambers of the resulting network $\cN_{\bD}(E_\inn,E_\out)$ are assigned the GS coordinates on $\P_{G,\Pi}$. We call $\cN_{\bD}(E_\inn,E_\out)$ the network associated with the pair $(E_\inn,E_\out)$ and the reduced words $\bs_1,\dots,\bs_M$. 
%A \emph{closed network path} in $\cN_{\bD}(E_\inn,E_\out)$ is a closed edge path obtained as a concatenation of network paths in the basic networks which traverses each basic network \emph{exactly once}. 
A \emph{network path} in $\cN_{\bD}(E_\inn,E_\out)$ is a concatenation of network paths in the basic networks, whose weight is defined to be the product of weights of the constituent paths in the basic networks. It is of type $(\alpha,\beta)$ for $\alpha,\beta \in \{1,\dots,\dim V\}$ if the first constituent path in $\cN_{\tau_M}(\lie,\bs_M)$ is of type $(\ast,\beta)$ and the last one in $\cN_{\tau_1}(\lie,\bs_1)$ is of type $(\alpha,\ast)$ for some $\ast \in \{1,\dots,\dim V\}$. The set of network paths in $\cN_{\bD}(E_\inn,E_\out)$ of type $(\alpha,\beta)$ is denoted by $P_{\alpha\beta}(E_\inn,E_\out)$. 

The following is our main theorem in this section. 

\begin{thm}[Network expansion formula for side pairings]\label{t:network formula}
Let $\Pi$ be a polygon equipped with an ideal triangulation $\Delta$, $(E_\inn,E_\out)$ a pair of its side edges, and $\tau_\Delta(E_\inn,E_\out)=(\tau_1,\dots,\tau_M)$ the associated turning pattern. Let $\bs_1,\dots,\bs_M$ be reduced words of $w_0$. Then in terms of the GS coordinates associated with $\bD:=(\Delta_*(E_\inn,E_\out),(\bs_\nu)_{\nu=1}^M)$, the matrix coefficients of the side pairing can be written as 
\begin{align*}
    \bra{\alpha}(\psi_{\bD}^+)^*g_{E_\inn,E_\out}^+\ket{\beta}= \sfh_{\lie}(\mathbb{X})\sum_{\omega \in P_{\alpha\beta}(E_\inn,E_\out)} wt_\omega(\bX).
\end{align*}
Here $\sfh_{\lie}(\mathbb{X}_{E_\inn,E_\out}):=\prod_{(s,i;\nu)\in I_1\ast \dots \ast I_M} X_i^s[\nu]^{-C^{s,1^\ast}}$.
\end{thm}

\begin{proof}
From \cref{l:positive_decomp} and the network expansion formulae in the previous subsection, we have
\begin{align*}
    (\alpha_{\bD}^+)^*\bra{\alpha} (\psi^+_{\bD})^*g_{E_\inn,E_\out}^+\ket{\beta} &= \bra{\alpha} (\dprod_{\nu=1}^M\psi_{\bs_\nu}^+)^*(q_\Delta^+)^*g_{E_\inn,E_\out}^+\ket{\beta} \\
    &=\sum_{\alpha_1,\dots,\alpha_{M-1}} \bra{\alpha}(\psi_{\bs_1}^+)^*b_{\tau_1}\ket{\alpha_1}\cdots \bra{\alpha_{M-1}}(\psi_{\bs_M}^+)^*b_{\tau_M}\ket{\beta} \\
    &=\sfh_{\lie}(\mathbb{X}_{E_\inn,E_\out})\sum_{\omega_1,\dots,\omega_M} wt_{\omega_1}\cdots wt_{\omega_{M}},
\end{align*}
where the last summation is over network paths $\omega_\nu \in P_{\alpha_{\nu-1}\alpha_\nu}^{\tau_\nu}$ for $\nu=1,\dots,M$ with $\alpha_0=\alpha$, $\alpha_M=\beta$. 
Since our assignment of GS coordinates on the chambers of the network $\cN_{\bD}(E_\inn,E_\out)$ is compatible with amalgamations and the paths $\omega_1,\dots,\omega_M$ in the summation above can be concatenated to form a network path in $\cN_{\bD}(E_\inn,E_\out)$ of type $(\alpha,\beta)$, we get the desired formula.
\end{proof}
In particular, the monomials in the positive Laurent polynomial $\bra{\alpha}(\psi_{\bD}^+)^*g_{E_\inn,E_\out}^+\ket{\beta}$ are parametrized by the network paths in $\cN_{\bD}(E_\inn,E_\out)$.

A generalization for Wilson lines and Wilson loops is now straightforward. Let $\Sigma$ be a marked surface equipped with a decorated triangulation $\bD$, $[c]:E_\inn \to E_\out$ a morphism in $\Pi_1^\partial(\Sigma)$. Recall the twisted chain $\hat{\bX}_{[c]}=(\hat{X}_i^s[\nu])$ of GS coordinates on $\P_{G,\Sigma}$ along $[c]$. 
Let $\cN_{\bD}([c])$ be the network obtained from $\cN_{\bD}(\widetilde{E}_\inn,\widetilde{E}_\out)$ by replacing each GS coordinate $X_i^s[\nu]$ assigned to chambers with $\hat{X}_i^s[\nu]$. The set $P_{\alpha\beta}([c])$ of network paths in $\cN_{\bD}([c])$ of type $(\alpha,\beta)$ as well as their weights are defined similarly.

\begin{cor}[Network expansion formula for Wilson lines]
Let $\Sigma$ be a marked surface equipped with a decorated triangulation $\bD$, $[c]:E_\inn \to E_\out$ a morphism in $\Pi_1^\partial(\Sigma)$. 
Then in terms of the GS coordinates associated with $\bD$, the matrix coefficients of the Wilson loop can be written as 
\begin{align*}
    \bra{\alpha}(\psi_{\bD}^+)^*g_{[c]}^+\ket{\beta}= \sfh_{\lie}(\hat{\mathbb{X}}_{[c]})\sum_{\omega \in P_{\alpha\beta}([c])} wt_\omega(\hat{\bX}_{[c]}).
\end{align*}
Here $\sfh_{\lie}(\hat{\mathbb{X}}_{[c]}):=\prod_{(s,i;\nu)\in I_1\ast \dots \ast I_M} \hat{X}_i^s[\nu]^{-C^{s,1^\ast}}$.
\end{cor}
Note that in general, it is no more true that each term $wt_\omega(\hat{\bX}_{[c]})$ is a monomial of GS coordinates as $\hat{X}_i^s[\nu]$ is not. 
We have the following two cases where it becomes a monomial:

\begin{description}
    \item[Simple triangulations]
    For a morphism $[c]: E_\inn \to E_\out$ in $\Pi_1^\partial(\Sigma)$, we say that an ideal triangulation $\Delta$ of $\Sigma$ is \emph{$[c]$-simple} if $[c]$ is represented by a path which intersects at most two edges of each triangle of $\Delta$. In particular one can choose a dotted triangulation $\Delta_*$ over $\Delta$ so that $\Delta_*^{\mathrm{can}} = \Delta_*^{\mathrm{lift}}$ on the polygon $\Pi_{c;\Delta}$. We call such a dotted triangulation \emph{$[c]$-compatible}. In this case we have $t_\nu=0$ for $\nu=1,\dots,M$, and hence each $\hat{X}_i^s[\nu]$ is a single GS coordinate associated with $\bD$. 
    \item[Type $A_n$]
    Recall from \cref{l:cyclic shift A_n} that the cyclic shift $\mathcal{S}_3$ just permute the GS coordinates on a triangle in type $A_n$ case. Hence each $\hat{X}_i^s[\nu]$ is a single GS coordinate associated with $\bD$ in this case.
\end{description}


\begin{cor}\label{c:mon_simple case}
Let $\bD$ be a decorated triangulation, $[c]: E_\inn \to E_\out$ a morphism, and the notations as above. Suppose either that the underlying triangulation $\Delta$ is $[c]$-simple or the Lie algebra $\lie$ is of type $A_n$. Then the weight $wt_\omega(\hat{\bX}_{[c]})$ of each network path $\omega\in P_{\alpha\beta}([c])$ is a monomial of GS coordinates on $\P_{G,\Sigma}$. 
\end{cor}
In particular, the monomials in the positive Laurent polynomial $\bra{\alpha}(\psi_{\bD}^+)^*g_{[c]}^+(\hat{\bX}_{[c]})\ket{\beta}$ is parametrized by networks paths in these cases. 

Finally, let $|\gamma| \in \hat{\pi}_1(\Sigma)$ be a free loop on a marked surface $\Sigma$ (possibly with empty boundary), $\bD$ a decorated triangulation. Recall the twisted cycle $\hat{\bX}_{|\gamma|}=(\hat{X}_i^s[\nu])$ of GS coordinates on $\P_{G,\Sigma}$ along $|\gamma|$. 
Let $\cN_{\bD}(|\gamma|)$ be the network obtained from $\cN_{\bD}(\widetilde{E}_\inn,\widetilde{E}_\out)$ by further concatenating the right endpoints of $\cN_{\tau_M}(\lie,\bs_M)$ to the left endpoints of $\cN_{\tau_1}(\lie,\bs_1)$ with the same basis labels, and then replacing each GS coordinate $X_i^s[\nu]$ assigned to chambers with $\hat{X}_i^s[\nu]$. A \emph{closed network path} is a concatenation of network paths in the basic networks which forms a closed path, whose weight is defined to be the product of weights of the constituent paths in the basic networks. 
Let $P_{\mathrm{cl}}(|\gamma|)$ be the set of closed network paths in $\cN_{\bD}(|\gamma|)$.

\begin{cor}[Network expansion formula for Wilson loops]
Let $\Sigma$ be a marked surface equipped with a decorated triangulation $\bD$, $|\gamma| \in \hat{\pi}_1(\Sigma)$ a free loop. 
Then in terms of the GS coordinates associated with $\bD$, the trace of the Wilson loop can be written as 
\begin{align*}
    \mathrm{tr}_V((\psi_{\bD}^+)^*\rho_{|\gamma|}^+)= \sfh_{\lie}(\hat{\mathbb{X}}_{|\gamma|})\sum_{\omega \in P_{\mathrm{cl}}(|\gamma|)} wt_\omega(\hat{\bX}_{|\gamma|}).
\end{align*}
Here $\sfh_{\lie}(\hat{\mathbb{X}}_{|\gamma|}):=\prod_{(s,i;\nu)\in I_1\ast \dots \ast I_M} \hat{X}_i^s[\nu]^{-C^{s,1^\ast}}$.
\end{cor}
A $|\gamma|$-simple ideal triangulation is similarly defined, and a result similar to \cref{c:mon_simple case} also holds.
